A posteriori error control for fourth-order semilinear problems with quadratic nonlinearity

A general a posteriori error analysis applies to five lowest-order finite element methods for two fourth-order semi-linear problems with trilinear non-linearity and a general source. A quasi-optimal smoother extends the source term to the discrete trial space, and more importantly, modifies the trilinear term in the stream-function vorticity formulation of the incompressible 2D Navier-Stokes and the von K\'{a}rm\'{a}n equations. This enables the first efficient and reliable a posteriori error estimates for the 2D Navier-Stokes equations in the stream-function vorticity formulation for Morley, two discontinuous Galerkin, $C^0$ interior penalty, and WOPSIP discretizations with piecewise quadratic polynomials.

==> sections/main_clean.tex <==

	\maketitle
\abstract{
%
%
%
%
A general  a posteriori error analysis applies to  five lowest-order finite element methods for  two fourth-order semi-linear problems with trilinear non-linearity and a general source.   A quasi-optimal smoother extends the source term to the discrete trial space, and more importantly, modifies the trilinear term in the stream-function vorticity formulation of the incompressible 2D Navier-Stokes and the  \vket.  This enables the first efficient and reliable a posteriori error estimates for the 2D Navier-Stokes equations in the stream-function vorticity formulation for
Morley, two discontinuous Galerkin, $C^0$ interior penalty, and WOPSIP discretizations with piecewise quadratic polynomials.}
	
\medskip
\noindent \textbf{Mathematics subject classification:} 
65N30,  65N12, 65N50.

\medskip 
\noindent \textbf{Keywords:} semilinear problems, nonsmooth data, a posteriori,  efficient, reliable, error control, smoother, Navier-Stokes, von K\'{a}rm\'{a}n, Morley, discontinuous Galerkin, $C^0$ interior penalty, WOPSIP.

	
	\section{Introduction}
	This paper discusses an abstract a posteriori error analysis for fourth-order semilinear problems and
	its applications to the incompressible 2D Navier-Stokes equations and the von K\'arm\'an equations.
The continuous problem in this paper seeks a regular root $u$ 
in a Banach space $X$   to $N \in C^1(X;Y^*)$ for
\begin{equation}\label{eqn:cont}
N (x):= a(x,\bullet) + {\Gamma}(x,x,\bullet)- F \text{ for } x \in X. 
\end{equation}
%
%
%
The bilinear form $a(\bullet,\bullet)$ in \eqref{eqn:cont} corresponds to a weak form of the biharmonic operator, the trilinear form $\Gamma(\bullet,\bullet,\bullet)$ represents a quadratic nonlinearity, and $F$ is the general source term in $Y^*$; for instance, for the 2D Navier-Stokes equations in the stream-function vorticity formulation and for the von K\'{a}rm\'{a}n plates. 
The nonconforming discretization of \eqref{eqn:cont} with a piecewise application of the differential operators in the weak forms for Morley finite element functions \cite{CCGMNN_semilinear} allows for a priori convergence results. But their a posteriori error analysis so far was not satisfactory for the stream-function vorticity formulation of the incompressible 2D Navier-Stokes equations \cite{CCGMNN_semilinear, kim_morley_2021}: the efficiency analysis is excluded in \cite{CCGMNN_semilinear} and merely partial in  \cite[Remark
 4.11]{kim_morley_2021}. 
 %
 For the (generalised) Morley interpolation operator $I_\M$, the companion operator $J$ \cite{aCCP, ccnnlower2022,CCBGNN22}, the smoother $J_h=JI_\M=S=Q$,  the  choice $R \in \{{\rm id}, I_{\M},  JI_\M\}$, 
 %
%
the discrete problem \cite{CCNNGRDS22} seeks an approximation $u_h$ to a regular root $u$ to \eqref{eqn:cont}   in  a finite-dimensional space $X_h$ as a root of 
\begin{equation}\label{eqn:discrete}
N_h(u_h) := \dislin(u_h,\bullet) + {\Gamma}_{\pw}(\rop u_h,\rop u_h,\sop\bullet)- F_h.%
\end{equation}
 The bilinear form $a_h(\bullet,\bullet)$  discretizes $a(\bullet,\bullet)$, for instance, with Morley \cite{DG_Morley_Eigen,CCDG14,CCDGJH14},  discontinuous Galerkin (dG) \cite{Georgoulis2009, Georgoulis2011,CCGMNN18}, $C^0 $ interior penalty (IP) \cite{BS05,BS_C0IP_VKE},  and WOPSIP \cite{BrenGudiSung10} schemes;  the trilinear form $\Gamma_{\pw}(\bullet,\bullet,\bullet)$ discretizes $\Gamma(\bullet,\bullet,\bullet)$ by the piecewise action of the differential operators,  $F_h= F \circ Q$ approximates $F$,  and $R$, $S$ denote quasi-optimal smoothers in the spirit of \cite{veeser1,veeser2,veeser3,CCBGNN22,ccnnlower2022,CCNNGRDS22}. The innovative point  in \eqref{eqn:discrete} is the application of smoothers $R$ and $S$ in the nonlinearity $\Gamma_{\pw}(Ru_h,R u_h, Sy_h)$.
 %
 %
 %
%
%
The prequel \cite{CCNNGRDS22} establishes an a priori analysis of this class of lowest-order finite element methods and a source term $F \in Y^*$ with the {first} best-approximation result for $S=Q=J_h$, namely 
\begin{align}\label{eqn:QO}
    \|u - u_h \|_{\widehat{X}} \le 
C_{\rm qo} \min_{x_h \in X_h} \|u - x_{h}\|_{\widehat{X}}.\tag{\bf QO}
\end{align}
Here and throughout this paper, the Banach spaces $(X_h,\|\bullet\|_{X_h})$ and $(X,\|\bullet\|_X$) are contained in a common superspace $(\widehat X, \|\bullet\|_{\widehat X})  $ with a norm $\|\bullet\|_{\widehat X}$ that extends $\|\bullet\|_{X_h}=(\|\bullet\|_{\widehat X})|_{X_h}$ and $\|\bullet\|_{X}=(\|\bullet\|_{\widehat X})|_{X}$.
  This paper presents the first reliable and efficient  a posteriori error analysis for those schemes and includes the {\it first} reliable and efficient a posteriori estimates for the lowest-order finite element schemes for the  2D Navier-Stokes equation in the stream-function vorticity formulation.
  %

\smallskip \noindent
%
%
%
%
%
%
%
%
%
%
%
%

\smallskip \noindent 
Section~\ref{sec:Abstract a posteriori error control} 
introduces an abstract framework of an a posteriori error control in Banach spaces $X$ and $Y$ as in \eqref{eqn:cont}-\eqref{eqn:discrete} that applies below  to five second-order schemes, namely the Morley, two dG, $C^0$IP, and WOPSIP. The outcome allows for rough source terms $F \in Y^*$ and provides reliable and efficient error control by the sum of three contributions. Given an approximation $v_h \in X_h$ to a local discrete solution $u_h \in X_h$ to $N_h(u_h)=0$ for \eqref{eqn:discrete} near an exact regular root $u \in X$ to \eqref{eqn:cont}, there is an algebraic error $\|u_h-v_h\|_{X_h}$ and an inconsistency error $\|v_h-Jv_h\|_{\widehat X}$ plus some intermediate residual $\rho(M)$.
Theorem~\ref{thm:apost} provides the equivalence of the error $\|u-v_h\|_{\widehat X}$ to
$$ \rho(M) + (1+M) \|v_h - Jv_h\|_{\widehat{X}} +M \|u_h-v_h\|_{X_h}$$
for any parameter $M \ge 0$. The underlying assumptions are phrased in a fairly general non-symmetric setting for rather general trilinear forms $\Gamma$ resp. $\Gamma_{\pw}$, and involve 
%
smallness assumptions on $\|u-u_h\|_{\widehat{X}} \le \varepsilon $ and $\|u_h-v_h\|_{X_h} \le \varrho$ that are guaranteed in the two applications to the stream-function vorticity formulation of the incompressible 2D Navier-Stokes and the  \vket~\cite{CCNNGRDS22}.
%
The provided a posteriori error analysis is generic and allows generalisations to other semilinear equations in future work.

\medskip \noindent Section~\ref{subsection:new} concerns the particular situation with $V=X=Y=H^2_0(\Omega)$ and {$V_h= X_h=Y_h \subseteq P_2(\T)$} for some triangulation $\T$ and a discrete norm $\|\bullet\|_h$ in $H^2(\T)$.
The arbitrary parameter $M$ in Theorem~\ref{thm:apost} becomes an upper bound of an interpolation operator $I_h: V \rightarrow V_h$ for the equivalence of $\rho(M)$  to an explicit residual-based a posteriori error estimator $\eta(\T) +\mu(\T)$ up to oscillations ${\rm osc}_k(F,\T)$.
%
The abstract parts of this paper in Section~\ref{sec:Abstract a posteriori error control} concludes with some remarks on the algebraic error $\|u_h-v_h\|_{V_h}$ in the context of the Newton-Kantorovich theorem and Section~\ref{subsection:new} illustrates the generality of the abstract results in Subsection~\ref{sec:algebraic}. In fact, given any approximation $v$ to the regular root $u$ of \eqref{eqn:cont}, that is a piecewise smooth function with respect to a triangulation $\T$ with $V_h \subset P_2(\T)$, the general Morley interpolation $I_\M$ and an adoption to $V_h$ (in case of $C^0$IP) leads to a postprocessed $v_h \in V_h$ that is close to $u$. If $\|u-v_h\|_{\widehat V}$ is sufficiently small, then \eqref{eqn:discrete} with $Q=S={J I_\M}$ provides a reference scheme such that Theorem~\ref{thm:apost} and \ref{thm:releff} provide a reliable and efficient estimate for $u-v_h$ (cf. Subsection~{2.5.2} for details).
%
%
Thus the a posteriori error analysis in this paper covers many more examples beyond the mandatory inexact solve in \eqref{eqn:discrete} or the computation of the discrete solution by a related scheme (e.g., without smoother for $R=S=Q={\rm id}$ in \eqref{eqn:discrete}).

\smallskip \noindent The application to the stream-function vorticity formulation of the incompressible 2D Navier-Stokes in Section~\ref{sec:nse}  enables the {\it first} explicit reliable and efficient residual-based a posteriori error estimates in this context and overcomes the gaps in \cite{CCGMNN_semilinear, kim_morley_2021}. The application to the \vket~in Section~\ref{sec:vke} also considers single forces in the source terms. %
%
%
%
%
%
%
%
%
%
Section~\ref{sec:Numerical experiments} presents the {\it first} numerical comparisons of the quadratic schemes and confirms the a priori equivalence results in \cite{CCNNGRDS22}. The associated adaptive mesh-refining recovers the optimal convergence rates.

\smallskip \noindent
%
Standard notation on  Lebesgue and Sobolev spaces, 
their norms, and $L^2$ scalar products applies throughout this paper;  $\|\bullet\|$ %
abbreviates the operator norm of a linear operator.  
%
%
%
The Hilbert space $V := H_0^2(\Omega)$ is endowed with the energy scalar product $a(\bullet,
\bullet)$ that induces
the $H^2$ seminorm $\displaystyle\trinl\bullet\trinr := |\bullet|_{H^2(\Omega)}$; the induced dual linear operator norm in $H^{-2}(\Omega)$ is denoted by $\trinl \bullet \trinr_{*}$ in the later sections. In the sequel, the notation $A \lesssim B$ abbreviates $A \leq CB$ for some positive generic constant $C$, 
which exclusively depends on the shape-regularity of the underlying triangulation $\T$ (i.e., on $0 < \omega_0 \le {\arcangle} {T}$),  
 $A\approx B$ abbreviates $A\lesssim B \lesssim A$. 
%
%
%
%
%
%
%
%
%
%
%
%
	%
%
%
%
%
%
%
%
%
%
%



%
%
%
%
%
%
%
%
%
%
%
%
%


 %
%
%


%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%

\section{Abstract a posteriori error analysis}\label{sec:Abstract a posteriori error control}
The a posteriori error analysis concerns some approximation $v_h \in X_h$ in some
discrete nonconforming space $X_h\not\subset X$ to a regular root $u$ of the continuous problem \eqref{eqn:cont}. The known approximation could result from an inexact solve of the discrete problem 
\eqref{eqn:discrete} with local solution $u_h \in X_h$; hence $u_h$ and $v_h$ are different in general and the main interest is on the distance of $u$ and $v_h$. The abstract results of this section also apply to semilinear second-order problems in future work. 
		
		\subsection{Discretisation}%
		\label{sub:Discretisation}
%
%
%
%

\noindent Let $\widehat{X}$ (resp. $\widehat{Y}$) be a real Banach space with norm $\|\bullet\|_{\widehat{X}}$ (resp.\ $\|\bullet\|_{\widehat{Y}}$) and suppose $X$ and $X_h$ (resp.\ $Y$ and $Y_h$) are two complete linear subspaces of $\widehat{X}$ (resp.\ $\widehat{Y}$) with inherited norms $\|\bullet\|_{X}:=\big(\|\bullet\|_{\widehat{X}}\big)|_{X}$ and $\|\bullet\|_{X_h}:=\big(\|\bullet\|_{\widehat{X}}\big)|_{X_h}$ (resp.\ $\|\bullet\|_{Y}:=\big(\|\bullet\|_{\widehat{Y}}\big)|_{Y}$ and $\|\bullet\|_{Y_h}:=\big(\|\bullet\|_{\widehat{Y}}\big)|_{Y_h}$){; $X + X_h \subseteq \widehat{X}$ and $Y + Y_h \subseteq \widehat{Y}$.} Let the bounded linear operator
${A}\in L({X}; {Y}^*)$ be associated to the 
bilinear form $a$ and suppose $A$ is invertible and, in particular, satisfies
%
\begin{gather} 
0 < \alpha :=\inf_{\substack{{x} \in {X} \\ \|{x}\|_{{X}}=1}} \sup_{\substack{{y}\in {Y}\\ \|{y}\|_{{Y}}=1}} a({x},{y}).
%
%
\label{cts_infsup}
\end{gather}
Let $ \Gamma_{\pw}:\widehat{X}\times \widehat{X}\times \widehat{Y}\to \R$
denote a bounded trilinear form that extends $\Gamma=\Gamma_{\pw}|_{X\times X\times Y}$ 
%
such that
%
$$\displaystyle \| \Gamma_{\pw}\|:=\| \Gamma_{\pw}\|_{\widehat{X}\times \widehat{X}\times \widehat{Y}}:=
\sup_{\substack{\widehat{x}\in \widehat{X}\\ \|\widehat{x}\|_{\widehat{X}}=1}}
\sup_{\substack{\widehat{\xi}\in \widehat{X}\\ \|\widehat{\xi}\|_{\widehat{X}}=1}}
\sup_{\substack{\widehat{y}\in \widehat{Y}\\ \|\widehat{y}\|_{\widehat{Y}}=1}}
\Gamma_{\pw}(\widehat{x},\widehat{\xi},\widehat{y})~<\infty\quad\text{and set}\quad\| \Gamma\|:=\| \Gamma\|_{{X}\times {X}\times {Y}}.$$
%
Define the quadratic function $N:X \rightarrow Y^*$ by \eqref{eqn:cont}.
A vector $u \in X$ is called a {\it regular root} of \eqref{eqn:cont},  if  $u$ solves $N(u)=0$
%
%
%
%
 and the Frech\'et derivative $DN(u)$ is a bijection and, in particular, fulfils 
 %
	%
\begin{gather} 
0<\beta:=\inf_{\substack{x\in X\\ \|x\|_{X}=1}} \sup_{\substack{y\in Y\\ \|y\|_{Y}=1}}\Big(a(x,y)+ {\Gamma}(u,x,y)+{\Gamma}(x,u,y)\Big).
\label{cts_infsup_b}
\end{gather}
%
%
Suppose that the bounded bilinear form $a_h:X_h \times Y_h \rightarrow {\mathbb R}$ suffices the discrete inf-sup condition
\begin{align} \label{eqn:stability}
&0 <  \alpha_h  :=\inf_{\substack{{x}_h\in {X}_h \\ \|{x_h}\|_{{X_h}}=1}} \sup_{\substack{{y}\in {Y_h}\\ \|{y_h}\|_{{Y}_h}=1}}\dislin({x_h},{y_h})
%
\end{align}
%
for some constant $\alpha_h$. 
%
%
%
%
%
%
%
%
The quasi-optimal smoothers are linear and bounded operators  $P \in L(X_h;X)$, $Q \in L(Y_h;Y)$,  $\rop \in L(X_h;\widehat{X})$, $S \in L(Y_h;
\widehat{Y})$ {with respective operator norms $\|P\|, \|Q\|, \|R\|$, and $\|S\|$}  such that, for all $x_h \in X_h, \: x \in X,\: y_h \in Y_h, $ and $y \in Y$,
\begin{align}
	\| (1 - P)x_h \|_{\widehat{X}} & \le \Lambda_{\rm P} \| x - x_h \|_{\widehat{X}}, \label{quasioptimalsmootherP}\\
	\| (1 - Q)y_h \|_{\widehat{Y}} & \le \Lambda_{\rm Q} \| y - y_h \|_{\widehat{Y}}, \label{quasioptimalsmootherQ}\\
	\| (1 - \rop)x_h \|_{\widehat{X}} & \le \lamr\| x - x_h \|_{\widehat{X}}, \label{quasioptimalsmootherR}\\
	\| (1 - \sop)y_h \|_{\widehat{Y}} & \le \lams\| y - y_h \|_{\widehat{Y}} \label{quasioptimalsmootherS}
 \end{align}
hold with constants $\Lambda_{\rm P},\Lambda_{\rm Q},  \lamr, \lams \ge 0$. Suppose there exists $\Lambda_{\rm C}>0$ such that
\begin{align}
 a(Px_h,Qy_h)- \dislin(x_h,y_h) & \le \Lambda_{\rm C} \| x_h - Px_h\|_{\widehat{X}} \| y_h \|_{Y_h} \label{eqn:H}
\end{align}
holds for all $(x_h,y_h) \in X_h \times Y_h$. While \eqref{eqn:stability} is stability, \eqref{eqn:H} is consistency introduced in \cite{ccnnlower2022} for linear problems. Let the quadratic function $N_h:X_h \rightarrow Y_h^*$ be defined by \eqref{eqn:discrete}. The local conditions on the roots $u$, $u_h$, and their approximation $v_h$ are summarised as follows. 
%
%
%
%
\begin{enumerate}
\item[{\bf (L)}]
 Let $u\in X$ denote a regular root of \eqref{eqn:cont} for a given source term $F \in  Y^*$ and
    let there exist $\varepsilon,\varrho >0$ and  {$0<\kappa <1$} such that
    \begin{itemize}
    \item[{\bf (L1)}]  $N_h(u_h)=0$  holds for exactly one solution $u_h\in X_h $  with $\| u-u_h\|_{\widehat{X}} \le \varepsilon$, 
    \item[{\bf (L2)}] $v_h \in X_h$ satisfies $\|u_h-v_h\|_{{X_h}}  \le \varrho$,
    \item[{\bf (L3)}] $\varepsilon+\varrho\leq\kappa\beta/\left((1+\LP)\|\Gamma\|\right)$.
    \end{itemize}
    \end{enumerate}
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
 %
%
%
%
%
%
 %
%
%
%
The point is that the recent paper \cite{CCNNGRDS22} provides affirmative examples for all those conditions \eqref{cts_infsup}-\eqref{eqn:H}, {\bf (L1)}-{\bf (L3)}, and \eqref{eqn:QO} with constants that are independent of some discretisation parameter {$h$}, provided the discretization is sufficiently fine.
\subsection{Abstract a posteriori analysis} 
\label{subsec:outline}

This section presents an  abstract reliability  and  efficiency result. %
The abstract a posteriori error control has three contributions. The first one is an  intermediate residual 
\begin{align} \label{a}
\displaystyle \rho(M)&:= \sup_{\stackrel{y \in Y}{\|y \|_Y \le 1} } \inf_{\stackrel{y_h \in Y_h}{\|y_h \|_{Y_h} \le M} }  %
\Big( F(y-Qy_h)-a(Pv_h,y-Qy_h) -
\Gamma_{\pw}(Rv_h, Rv_h, y-Sy_h)  \Big)
\end{align}
for some parameter $M \ge 0$. The role of $M$ will be clarified in Section~\ref{subsection:new} below. At this point it suffices to observe that $y_h$ may be some discrete object such that $Qy_h$ and $Sy_h$ approximate $y$ and we expect
$\|y_h\|_{Y_h} \le M \|y\|_{Y} \le M$ is bounded.  Notice that $\rho$ is monotone decreasing and $\rho(0) \ge \rho(M)$. %
The second contribution is a consistency term $\|v_h-Pv_h\|_{\widehat{X} }$ (computable from $v_h \in X_h$ and
the quasi-optimal smoother $P$) with \eqref{quasioptimalsmootherP} and throughout serves as an efficient a posteriori term
\cite{CCBGNN22}. The third term $\|u_h-v_h\|_{X_h} \le \varrho$ is the algebraic error (e.g., from an inexact solve) and  is briefly discussed in Subsection~\ref{sec:algebraic}.
%
%
%
%
%
\begin{theorem}[abstract reliability and efficiency]\label{thm:apost}
	(a) Suppose {\bf (L1)}--{\bf (L3)}, \eqref{quasioptimalsmootherP}-\eqref{quasioptimalsmootherR}, \eqref{eqn:H}, and $M \ge 0$. Then 
 %
%
%
%
%
%
%
%
\begin{align}
  & \displaystyle \| u- v_h\|_{\widehat{X}}  \le
%
%
%
C_{\rm rel} \Big( \rho(M)  + (1+M) \|(1-P)v_h\|_{\widehat{X}} +M\|u_h-v_h\|_{X_h} \Big). %
 \label{eqn:apost} %
\end{align}
%
The  constant  $C_{\rm rel} $  %
exclusively depends on  $\beta, (1-\kappa)^{-1}, \Lambda_{\rm C}, \Lambda_{\rm P},$ $ \Lambda_{\rm R}, \|a_h\|, $ $ \|\Gamma\|,\|\Gamma_\pw\|,\|S\|,$ and $\|u\|_{X}$.

\medskip \noindent 
(b) Suppose {\bf (L1)}--{\bf (L2)} and \eqref{eqn:QO}. Then $\rho(M) \le \rho(0)$ and
\begin{align} \label{eq:eff}
& \rho(0)  +\|(1-P)v_h\|_{\widehat{X}} +\|u_h-v_h\|_{X_h} 
 \le C_{\rm eff}\| u- v_h\|_{\widehat{X}}. 
 \end{align}
 The  constant  $C_{\rm eff} $  %
exclusively depends on $ \beta, (1-\kappa)^{-1}, \Lambda_{\rm C},\Lambda_{\rm P}, \Lambda_{\rm R}, \|a_h\|,  \|\Gamma\|,\|\Gamma_\pw\|,\|S\|,\|u\|_{X}$, and $C_{\rm qo}$.
\end{theorem}

%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%


\subsection{Proof of Theorem~\ref{thm:apost}.a}
	\label{sec:apost}
The proof is split into several subsections below with $u$, $u_h$, $v_h$ as in the statement of Theorem~\ref{thm:apost}.
%
%
%
%
%
%
%
\subsubsection{Reduction to $\|u-Pv_h\|_X$}\label{step1}
Consequences of  \eqref{quasioptimalsmootherP}, \eqref{quasioptimalsmootherR},  and a  triangle inequality read, for 
%
 any
$x\in X$ and $x_h \in X_h$, as
\begin{align} 
\|v_h-Pv_h\|_{\widehat{X}} &\le  \Lambda_{\rm P} \|u-v_h\|_{\widehat{X}}, \label{eqn:vh-Pvh} \\
 \|x- Px_h\|_{{X}} &\le (1+\Lambda_{\rm P}) \|x-x_h\|_{\widehat{X}},  \label{eqn:PR1} \\
\|x- Rx_h\|_{\widehat{X}} &\le (1+\Lambda_{\rm R}) \|x-x_h\|_{\widehat{X}},  \label{eqn:PR2} \\
 \| (P-R)x_h\|_{\widehat{X}} & \le (1+\Lambda_{\rm R}) \|  x_h- Px_h\|_{\widehat{X}}. \label{eqn:PR3}
\end{align}
%
%
%
%
The efficiency \eqref{eqn:vh-Pvh} of the  a posteriori estimator $\|v_h-Pv_h\|_{\widehat{X}}$ and a triangle inequality 
	\begin{equation}\label{eq.tri.rel}
	\|u-v_h\|_{\widehat{X}} \le \|u-Pv_h\|_{{X}}+\|v_h-Pv_h\|_{\widehat{X}} 
	\end{equation}
motivate the focus on $\|u-Pv_h\|_{{X}}$ in the error analysis below.
%
\subsubsection{Reduction to $ \| N(Pv_h)\|_{Y^*}$}
%
 %
%
	The inf-sup condition \eqref{cts_infsup_b} with $\beta>0$  for the regular root $u$ %
 leads, for any $\tau>0$, to
some $y\in Y$ with $\|y\|_{Y}\le 1+\tau$  and 
	\begin{equation}\label{Der_infsup}
	\beta \|u-Pv_h\|_{X} =  DN(u;Pv_h-u,y).
	\end{equation}
 (For reflexive Banach spaces, $\tau=0$ is possible, but for the time being we require $\tau>0$). 
	Since $N$ is quadratic, the finite Taylor series is exact, namely
	\begin{align*}%
	N(Pv_h;y)=N(u;y)+DN(u;Pv_h-u,y)+\half D^2N(u;u-Pv_h,u-Pv_h,y).
	\end{align*}
	Since $N(u)=0$ and $D^2N(u;u-Pv_h,u-Pv_h,y)=2 \, \Gamma(u-Pv_h,u-Pv_h,y)$, this reads 
	\begin{align}\label{quadratic_identity}
	N(Pv_h;y)+DN(u;u-Pv_h,y)& =  \Gamma(u-Pv_h,u-Pv_h,y).
	\end{align}
	The combination of \eqref{Der_infsup}-\eqref{quadratic_identity} and the bound $\|\Gamma\|$ of the trilinear form result in 
%
	\begin{align}\label{eqn:newa}
{\beta}  \|u-Pv_h\|_{X}& %
	%
	\leq \big(\| N(Pv_h)\|_{Y^*} + \|\Gamma\| \|u-Pv_h\|^2_{X}\big) (1+\tau)
	\end{align}
	with $\|y\|_{Y} \le 1+\tau$ in the last step. 
	%
Recall that \eqref{eqn:newa} holds for any $\tau>0$ and so $\tau \searrow0 $ provides
\begin{align} \label{eqn:new}
{\beta}  \|u-Pv_h\|_{X}& \le \| N(Pv_h)\|_{Y^*} + \|\Gamma\| \|u-Pv_h\|^2_{X}.
%
%
%
%
%
 %
%
%
%
%
%
%
\end{align}
%
%
%
%
Since $\|u-Pv_h\|_{X} \le (1+\Lambda_{\rm P}) \|u-v_h\|_{\widehat{X}}$ by \eqref{eqn:PR1} and
$\|u-v_h\|_{\widehat{X}} \le \|u-u_h\|_{\widehat{X}} + 
\|u_h-v_h\|_{X_h} \le \varepsilon + \varrho$ by {\bf (L1)}-{\bf (L2)}, we infer
$$ \|\Gamma \| \|u-Pv_h\|_{X} \le 
 \|\Gamma \| (1+\Lambda_{\rm P}) (\varepsilon + \varrho) \le \kappa \beta$$ with  {\bf (L3)} in the last step. This and \eqref{eqn:new} imply
 \begin{align} \label{eqn:bounda}
 \beta (1-\kappa) \|u-Pv_h\|_{X}
 & \le \|N(Pv_h)\|_{Y^*}.
 \end{align}
 The combination of \eqref{eq.tri.rel} and \eqref{eqn:bounda} reveals
 \begin{align} \label{eqn:u-vh}
    \|u-v_h\|_{\widehat{X}} & \le 
     \|v_h -Pv_h\|_{\widehat{X}}+
    \beta^{-1} (1-\kappa)^{-1} \|N(Pv_h)\|_{Y^*}
 \end{align}
 and we are left with the a posteriori analysis of $\|N(Pv_h)\|_{Y^*}$.
\subsubsection{Appearance of $\rho(M)$}\label{sub:varrho} To control $\| N(Pv_h)\|_{Y^*}$, consider any $y \in Y$ with $\|y\|_{Y} =1$
and any $y_h \in Y_h$ with $\|y_h\|_{Y_h} \le M$. 
Elementary algebra with the definition of $N(Pv_h; y)$ leads to
\begin{align} \label{eqn:newb}
	N(Pv_h; y)& = a(Pv_h,y-Qy_h) + \Gamma_{\pw}(Rv_h,Rv_h, y-Sy_h) -{F}(y-Qy_h) \nonumber \\
	& \quad + \Gamma_{\pw}(Pv_h,Pv_h,y) -\Gamma_{\pw}(Rv_h,Rv_h, y)  
	\nonumber \\
	& \quad  +a(Pv_h,Qy_h)-F(Qy_h) + \Gamma_{\pw}(Rv_h,Rv_h, Sy_h) =:S_1+S_2+S_3.
%
\end{align}
The  first  term  $S_1$ %
 gives rise to the intermediate residual 
$$
S_1:=a(Pv_h,y-Qy_h) + \Gamma_{\pw}(Rv_h,Rv_h, y-Sy_h) -{F}(y-Qy_h) \le \rho(M) $$
provided $y_h \in Y_h$ is selected to obtain an infimum in \eqref{a}. \big(The analysis of the remaining terms $ S_2+S_3 $ exclusively utilizes  $y_h \in Y_h$ and $\|y_h\|_{Y_h} \le M$  below.\big) Thus
\begin{align}\label{eqn:intermediate}
N(Pv_h; y)
 \le  \rho(M) + S_2+S_3. 
 \end{align}
%
%
%
%
\subsubsection{Difference of the trilinear form $S_2$}\label{S2}
Elementary algebra and the boundedness  of the piecewise trilinear form result in 
\begin{align} \label{t2}
S_2 & :=\Gamma_{\pw}(Pv_h,Pv_h,y) -\Gamma_{\pw}(Rv_h,Rv_h, y)   \nonumber \\
&= \Gamma_{\pw}((P-R)v_h,Pv_h,y) +\Gamma_{\pw}(Rv_h,(P-R)v_h, y) \nonumber \\
& \le \|\Gamma_\pw\|  (1+\Lambda_{\rm R}) (\|P\|+ \|R\|) \|v_h\|_{X_h} \|v_h-Pv_h \|_{\widehat{X}}
\end{align}
with \eqref{eqn:PR3} and $\| y\|_Y {=1}$  in the last step.

\medskip \noindent 
All the operator norms $\|P\|, \|Q\|, \|R\|, \|S\|$ of the quasi-optimal smoothers are controlled in terms of  $\Lambda_{\rm P}$, $\Lambda_{\rm Q}$,  $\Lambda_{\rm R}$, and  $\Lambda_{\rm S}$. For instance, \eqref{quasioptimalsmootherR} shows  $\|Rv_h\|_{\widehat{X}} \le (1+\Lambda_{\rm R})  \|v_h\|_{X_h}$.
%
%
%
%
%
  \subsubsection{Remaining bound $S_3$}
The last term $ S_3$ on the right-hand side of \eqref{eqn:newb} reads 
$$S_3:= a(Pv_h,Qy_h)-F(Qy_h) + \Gamma_{\pw}(Rv_h,Rv_h, Sy_h).$$
A comparison with
$N_h(u_h;y_h)=0$ from \eqref{eqn:discrete} and elementary algebra result in 
\begin{align}\label{eqn:s3}
 S_3&= a(Pv_h,Qy_h)- a_h(v_h,y_h ) + a_h(v_h-u_h,y_h) \nonumber \\
 & \qquad + \Gamma_{\pw}(Rv_h,Rv_h, Sy_h) - \Gamma_{\pw}(Ru_h,Ru_h, Sy_h).
 \end{align}
The consistency \eqref{eqn:H} controls the first two terms in the right-hand side of \eqref{eqn:s3},
\begin{align}\label{eqn:H_application}
a(Pv_h,Qy_h)- a_h(v_h,y_h ) & \le \Lambda_{\rm C} \|v_h-Pv_h\|_{\widehat{X}} \|y_h\|_{Y_h}.
\end{align}
The boundedness of $a_h$ establishes 
%
$a_h(v_h-u_h,y_h) \le \|a_h\|\|v_h-u_h\|_{X_h} \|y_h\|_{Y_h}.$
 %
Elementary algebra  for the last two terms in \eqref{eqn:s3} provides
%
 %
  %
  %
  %
\begin{align} \label{eqn:t2a}
& \Gamma_{\pw}(Rv_h,Rv_h, Sy_h) - \Gamma_{\pw}(Ru_h,Ru_h, Sy_h)  \nonumber \\
& =\Gamma_{\pw}(R(v_h-u_h),Rv_h, Sy_h)  + \Gamma_{\pw}(Ru_h,R(v_h-u_h), Sy_h)  \nonumber \\
 &  \le 
  \|\Gamma_\pw\|   \|R\|^2 \|S\| \Big( \|v_h\|_{X_h} +\|u_h\|_{X_h} \Big)  
   \|u_h-v_h\|_{X_h} \|y_h\|_{Y_h}
  \end{align}
  with boundedness of the piecewise trilinear form in the last step. 
A combination of the aforementioned  estimates with \eqref{eqn:s3} and $\|y_h\|_{Y_h} \le M$  shows
\begin{align}\label{eqn:s3a}
S_3 & \le M \Lambda_{\rm C} \|v_h-Pv_h\|_{\widehat{X}} + M\Big( \|a_h\|  + \|\Gamma_\pw\|   \|R\|^2 \|S\|  \big( \|v_h\|_{X_h} +\|u_h\|_{X_h} \big)  \Big)  \|u_h-v_h\|_{X_h}.
\end{align}
\subsubsection{Final a posteriori error estimate}\label{ssub:abstract_reliability_final}
Since $y \in Y$ with $\|y\|_Y =1$ is arbitrary, the combination of \eqref{t2} and \eqref{eqn:s3a} in \eqref{eqn:intermediate} leads to 
\begin{align}
\|N(Pv_h)\|_{Y^*} & \le \rho(M) + \Big(M \Lambda_{\rm C}  + \|\Gamma_\pw\|  \left(1+\Lambda_{\rm R} \right) \left(\|P\|+ \|R\|\right) \|v_h\|_{X_h}\Big) \|v_h-Pv_h\|_{\widehat{X}} \nonumber \\
& \qquad + M \Big( 
\|a_h\| + \|\Gamma_\pw\|   \|R\|^2 \|S\| 
\big( \|v_h\|_{X_h} +\|u_h\|_{X_h} \big)
 \Big) \|u_h-v_h\|_{X_h}.  \label{eqn:npvh}
\end{align}
%
%
Triangle inequalities and {\bf (L1)}-{\bf (L3)} reveal 
\begin{align} \label{eqn:vhbound}
\|v_h\|_{X_h} &\le \|u\|_X + \|u-u_h\|_{\widehat{X}} +\|u_h-v_h\|_{X_h} \le\|u\|_{X} + \varepsilon + \varrho  \le \|u\|_{X} +  \beta/ ((1+\Lambda_{\rm P}) \|\Gamma\|).
%
\end{align}
The same arguments apply to show $\|u_h\|_{X_h} \le \|u\|_X + \|u-u_h\|_{\widehat{X}} \le \|u\|_{X} +  \beta/ ((1+\Lambda_{\rm P}) \|\Gamma\|)$.
 A substitution of \eqref{eqn:vhbound} and the analog estimate for $\|u_h\|_{X_h}$ in 
\eqref{eqn:npvh} reveal
\begin{align}\label{eqn:ta}
\|N(Pv_h)\|_{Y^*}  \le \rho(M) + (M\Lambda_{\rm C} + C_1)  \|v_h-Pv_h\|_{\widehat{X}}  +C_2 M \|u_h-v_h\|_{X_h}
\end{align}
with  universal constants $\constant{}\label{ct4}:= 
\|\Gamma_\pw\|  \left(1+\Lambda_{\rm R} \right) \left(\|P\|+ \|R\|\right) \big(\|u\|_X+ \beta/ \big((1+\Lambda_{\rm P}) \|\Gamma\| \big) \big)$ and $\constant{} \label{ct5}:=
 \|a_h\| + 2\|\Gamma_\pw\|   \|R\|^2 \|S\|   \big(\|u\|_X+ \beta/ \big((1+\Lambda_{\rm P}) \|\Gamma\| \big) \big)
 $.
 %
A combination \eqref{eqn:ta} with \eqref{eqn:u-vh} provides
\begin{align} \label{eqn:est1}
\beta(1-\kappa) \|u-v_h\|_{\widehat{X}
 }& \le   \rho(M) + C_3 (1+M)\|v_h-Pv_h\|_{\widehat{X}}  +C_2 M\|u_h-v_h\|_{X_h}
\end{align}
with $\constant{}\label{ct3} := \max \big{\{} \Lambda_{\rm C}, C_1+\beta(1-\kappa) \big{\}} $. This concludes the proof of reliability with a reliability constant 
$C_{\rm rel}:= \beta^{-1}(1-\kappa)^{-1}\max \big{\{} 1, C_2 M, C_3 (1+M)\big{\}} $. \qed
%
%
%
%
%
%
%
%
%
%
%
%
 %
%
%
%
%
 %
%
%
\subsection{Proof of Theorem~\ref{thm:apost}.b}\label{sec:eff}
The efficiency of $\|v_h-Pv_h\|_{\widehat{X}}$ 
follows from \eqref{eqn:vh-Pvh} and hence the focus is on the other two terms $\rho(M)\leq\rho(0)$ and $\|u_h-v_h\|_{X_h}$.
\subsubsection{Linear intermediate problem}
%
%
The link between $\rho(M)$ from \eqref{a} to the known a posteriori results for linear problems reviewed in \cite{CCBGNN22} is the linear intermediate problem
\begin{align}\label{c}
a(\widetilde{u},y)&=F(y) - \Gamma_{\pw}(Rv_h,Rv_h,y)  \text{  for all } y \in Y.
\end{align}
Since the associated operator $A:X\to Y^*$ is invertible, the problem \eqref{c} admits a unique
solution $\widetilde u\in X$.
It follows that 
\begin{align}\label{d}
 \rho(M) & \le \rho(0)=   \sup_{\stackrel{y \in Y}{\|y \|_Y \le 1} } a(\widetilde{u}-Pv_h,y) \le \|a\| \: \|\widetilde{u} -Pv_h\|_{X}.
 \end{align} 
%
%
%
%
%
%
%
%
%
%
%
\subsubsection{Efficiency of $ \|u-\widetilde{u} \|_{X}$}
%
Recall that $u$ is a fixed regular root of $N$, while $\widetilde{u}$ solves 
\eqref{c}.  %
%
 %
%
%
%
%
 %
%
%
%
The inf-sup condition in \eqref{cts_infsup} leads,  for any $\tau>0$, to some  $ y \in Y$  with $\|y\|_Y \le 1+\tau$ and 
\begin{align*} 
\alpha \|u-\widetilde{u}\|_X &= a(\widetilde{u}-u,y) = \Gamma(u,u,y) -\Gamma_{\pw}(Rv_h,Rv_h,y )%
%
%
 %
\end{align*}
with \eqref{eqn:cont}  and \eqref{c} in the last step. This, the boundedness of the trilinear form, $\|u-Rv_h\|_{\widehat{X}} \le (1+\Lambda_{\rm R}) \|u-v_h\|_{\widehat{X}}$ from  \eqref{eqn:PR2}, and $\|y\|_Y \le 1+\tau$  provide
\begin{align*} 
\alpha \|u-\widetilde{u}\|_X &=\Gamma_{\pw}(u-Rv_h,u,y ) + \Gamma_{\pw}(Rv_h,u-Rv_h,y ) \nonumber \\
& 
 \le  \|\Gamma_\pw\| (1+\tau) (1+\Lambda_{\rm R}) \|u -v_h\|_{\widehat{X}} (\|u\|_X + \|Rv_h\|_{\widehat{X}}).
\end{align*}
The aforementioned estimate holds for any $\tau>0$, hence $\tau \searrow0 $ and  %
\eqref{eqn:vhbound} establish
%
%
%
\begin{equation} \label{eqn:u-ut}
 \|u- \widetilde{u}\|_{X} \le %
 \alpha^{-1} \|\Gamma_\pw\|  (1+\Lambda_{\rm R}) \Big(\|u\|_X + \|R\| \big(\|u\|_X +  \beta/ ((1+\Lambda_{\rm P}) \|\Gamma\|) \big)   \Big) \|u-v_h\|_{\widehat{X}}.
 \end{equation}
%
%
%
%
%
%
%
%
%
%
%
\subsubsection{Efficiency of $\rho(M)$}The intermediate problem \eqref{c} leads to 
\eqref{d}, namely 
\begin{align}\label{a1}
\rho(M) \le\rho(0) %
%
& \le \| a\| \| \widetilde{u} -Pv_h\|_{\widehat{X}} \le \|a\| \left(\|u - \widetilde{u}\|_X+ \|u-Pv_h\|_{X}\right).
\end{align}
Recall $\| u -Pv_h\|_{\widehat{X}} \le (1+\Lambda_{\rm P}) \| u -v_h\|_{\widehat{X}}$ from \eqref{eqn:PR1} and combine it with  \eqref{eqn:u-ut}-\eqref{a1} to deduce
%
%
%
%
%
%
%
%
%
$$\rho(0)  \le \|a\|\bigg(1+ \Lambda_{\rm P} +\alpha^{-1} \|\Gamma_\pw\|  (1+\Lambda_{\rm R}) \Big(\|u\|_X + \|R\| \big(\|u\|_X +  \beta/ ((1+\Lambda_{\rm P}) \|\Gamma\|) \big)   \Big)\bigg) \|u-v_h\|_{\widehat{X}}. \qed$$
%
%
%
%
\subsubsection
{Efficiency of $\|u_h-v_h\|_{X_h}$ under \eqref{eqn:QO}}  The quasi-best approximation \eqref{eqn:QO} implies $\|u-u_h\|_{\widehat{X}} \le C_{\rm qo} \|u-v_h\|_{\widehat{X}}$. This and a triangle inequality provide
$ \|u_h-v_h\|_{X_h} \le \|u-u_h\|_{\widehat{X}} + \|u-v_h\|_{\widehat{X}} \le (1+C_{\rm qo})\|u-v_h\|_{\widehat{X}}.$ \qed
%
%
%
 %


%
%
%
%
%
%
%
%
%



\subsection{Comments}

\subsubsection{Inexact solve}
%
The ad hoc application of Theorem~\ref{thm:apost} is on \eqref{eqn:discrete} with $S=Q$ and a flexible choice of $R$ with \eqref{quasioptimalsmootherR}. The local convergence of the Newton scheme is guaranteed in \cite{CCNNGRDS22} and a termination leads to $v_h \in X_h$ with an algebraic error discussed in Subsection~\ref{sec:algebraic} below. 
%
%
A few iterations more 
 provide the discrete solution up to machine precision and $\|u_h-v_h\|_h$ is negligible and this point of view is adapted in Section~\ref{sec:Numerical experiments}. %
 %
 %
%
%
%
%
%
%
%
%
\subsubsection{Approximation $v_h$ from other discretisations}
\label{sub:Approximation from other discretisations}
%
The discrete scheme in \eqref{eqn:discrete} with smoother $S=Q$ for the definition of $N_h$ in \eqref{eqn:discrete} and its root $u_h \in X_h$ with $\|u-u_h\|_{\widehat{X}} \le \varepsilon$ from {\bf(L1)} can serve as a reference scheme. Given an accurate approximation $v_h  \in X_h$ from another  numerical scheme that is sufficiently good in the sense that
\begin{equation}\label{eqn:varepsilon}
\|u-v_h\|_{\widehat{X}} \le \min \left\{\varepsilon,  {\varrho}/{(1+ C_{\rm qo})} \right\}.
\end{equation}
Since \eqref{eqn:QO} provides $\|u-u_h\|_{\widehat{X}} \le C_{\rm qo} \|u-v_h\|_{\widehat{X}}$, a triangle inequality and \eqref{eqn:varepsilon} reveal
\[  \| u_h-v_h\|_{X_h} \le (1+C_{\rm qo}) \| u-v_h\|_{\widehat{X}} \le \varrho.\]
%
%
Hence Theorem~\ref{thm:apost} applies to $v_h \in X_h$ and the explicit residual-based a posteriori estimators $\eta + \mu$ of Subsection~\ref{subsection:new}  lead to reliable and efficient error control of $\| u-v_h\|_{\widehat{X}} $. Although $v_h$ may originate from a very different setting, its a posteriori error control, namely the evaluation of $\| u-v_h\|_{\widehat{X}}$ in Theorem~\ref{thm:apost}, concerns the reference scheme $N_h$ from \eqref{eqn:discrete} with  $S=Q$.
%

\subsubsection{Control of algebraic errors}\label{sec:algebraic}
%
%
%
%
%
{The numerical analysis of the discrete problem as a high-dimensional algebraic system of equations %
%
is a routine task, e.g., with the known Newton scheme and the Newton-Kantorovich theorem. For instance, suppose that 
 $DN(u_h)$ satisfies the discrete inf-sup condition
\begin{align} \label{eqn:discreteinfsup}
0< \beta_h:=\inf_{\substack{x_h\in X_h\\ \|x_h\|_{X_h}=1}} \sup_{\substack{y_h\in Y_h\\ \|y_h\|_{Y}=1}}\Big(a_h(x_h,y_h)+ {\Gamma}_{\pw}(u_h,x_h,y_h)+{\Gamma}_{\pw}(x_h,u_h,y_h)\Big)
\end{align}
proved in  \cite{CCNNGRDS22} and recall that $u_h\in X_h$ is a discrete root of \eqref{eqn:discrete}. 
\begin{lemma}[control of $\|u_h-v_h\|_{X_h}$]\label{lem:uh-vh} Any $v_h\in X_h$ and $0<\kappa<1$ with $\|u_h-v_h\|_{X_h}\leq \kappa\beta_h/\big(\|\Gamma_\pw\|\|R\|^2\|S\|\big)$ satisfy
	\begin{align*}
		(1-\kappa)\beta_h\|u_h-v_h\|_{X_h} \leq \|N_h(v_h)\|_{Y_h^*}\leq \big(\kappa\beta_h +
		\|DN_h(u_h)\|_{X_h^*\times Y_h^*}\big)\|u_h-v_h\|_{X_h}.
	\end{align*}
\end{lemma}
\noindent The lemma is proved in Supplement A and an associated  termination criterion is outlined in Supplement~C.
\begin{example}[Computation of  $\|N_h(v_h)\|_{Y_h^*}$] \label{ex:computation_residual}If 
${\rm dim}(X_h)= {\rm dim}(Y_h) < \infty$ and 
\eqref{eqn:stability} holds, the linear operator $A_h : X_h \rightarrow Y_h^*$ associated with the bilinear form $a_h: X_h \times Y_h \rightarrow {\mathbb R}$ is invertible with  $\|A_h\|_{L(X_h; Y_h^*)}\|A_h^{-1}\|_{L(Y_h^*; X_h)} \le \|a_h\|/\alpha_h.$ Hence one linear solve of 
$a_h(\xi_h, y_h) =N_h(v_h; y_h)$ for a unique discrete solution $\xi_h \in X_h$ suffices for $\alpha_h \|\xi_h\|_{X_h} \le \|N_h(v_h)\|_{Y_h^*} \le \|a_h\| \|\xi_h\|_{X_h}$ and makes Lemma~\ref{lem:uh-vh} applicable.
\end{example}
%
\section{Explicit residual-based a posteriori estimator}\label{subsection:new}
This section discusses computable and explicit bounds for the intermediate residual $\rho(M)$ (and the consistency term $\|v_h-Pv_h\|_{X_h}$) in the reliablity control of Theorem \ref{thm:apost} in an application to fourth-order semilinear problems.
\subsection{Triangulation, interpolation, and smoother}\label{sub:triangulation, interpolation, and smoother}
 %
%
%
Throughout this paper, $\T$ denotes a shape-regular triangulation of a polygonal and bounded (possibly
multiply-connected) Lipschitz domain $\Omega\subset \mathbb
R^2$ into
triangles. The set of all  vertices $\mathcal{V}$ (resp.\ edges $\E$)  in the triangulation $\cT$  decomposes into interior vertices  $\mathcal{V}(\Omega)$ (resp.\ interior edges $\cE(\Omega)$) and boundary vertices  $\mathcal{V} (\partial\Omega)$ (resp.\ boundary edges $\cE(\partial\Omega)$).
Let $h_E\coloneqq |E|\coloneqq\mathrm{diam}(E)=|A-B|$ denote the length of any edge $E=\mathrm{conv}(A,B)\in\E$ with vertices $\mathcal V(E)=\{A,B\}$.
Define the piecewise constant mesh size $h_{\cT}(x)=h_T={\rm diam}  (T)$ for all $x \in T\in \cT$ (resp. $h_{\cE}(x)=h_E={\rm diam}  (E)$ for all $x \in E \in \cE$), and set $h_{\rm max} :=\max_{T\in \cT}h_T$.
The notation $\bT(\delta)$ denotes a family of  those triangulations $\T$ with maximal-mesh size $h_{\rm max}\leq\delta$ smaller than or equal to $\delta>0$ and interior angles $\ge \omega_0 >0$ for some universal constant $\omega_0$. 

The space $P_{\hspace{-.13em}k}(T)$ of polynomials of total degree at most $k\in\mathbb N_0$ on $T\in\T$ defines
the space of piecewise polynomials
\begin{align*}
	P_{\hspace{-.13em}k}(\T)&\coloneqq\{p\in L^\infty(\Omega) : p|_{T}\in P_{\hspace{-.13em}k}(T)\text{ for all } T\in \T\}
\end{align*}
and let $\Pi_k$ denote the $L^2$ projection onto $P_k(\T)$; $\Pi_k$ acts componentwise on vectors or matrices. Here and throughout this paper, $H^m(\T)\coloneqq \prod_{T\in\T}H^m(T)$ is the space of piecewise Sobolev functions for $m=1,2$ with the abbreviation $H^m(K)\coloneqq
H^m(\mathrm{int}\;K)$ for a triangle or edge $K\in \T\cup \E$ with relative interior $\mathrm{int}(K)$.
Let $H^m(\Omega; X),
H^m(\T; X)$, resp.~$P_{\hspace{-.13em}k}(\T; X)$ denote the space of (piecewise) Sobolev functions resp.~polynomials with values
in $X=\mathbb R^2, \mathbb R^{2\times2}, \mathbb S\subset\mathbb R^{2\times2}$ (symmetric $2 \times 2$ matrices).


%
%
%

Let $\nabla_\pw\coloneqq D_\pw$, $D^2_\pw$, and $\div_\pw$ denote the piecewise gradient, Hessian, and divergence operators without explicit reference to the underlying triangulation $\T$.
Notice that 
 $ (H^2(\cT), a_\pw+j_h)$ becomes a Hilbert space~\cite[Sec.~4]{CCBGNN22} with
 the scalar product 
 $a_\pw+ j_h:H^2(\T)\times H^2(\T)\to \mathbb R$ defined by
\begin{align} 
a_\pw(v_\pw,w_\pw)&\coloneqq(D^2_\pw v_\pw, D^2_\pw w_\pw)_{L^2(\Omega)}\qquad\text{for any }v_\pw,w_\pw\in H^2(\T),\label{eqn:a_pw_def}\\
	j_h(v_{\pw},w_\pw)&\coloneqq
	\sum_{E \in \E}\left( \sum_{z \in {\mathcal V} (E)} \frac{[v_{\pw}]_E(z)}{h_E}\frac{[w_\pw]_E(z)}{h_E}
			 +
\fint_E  \jump{\frac{\partial v_{\pw}}{\partial\nu_E}}_E\mathrm ds\, \fint_E  \jump{\frac{\partial w_\pw}{\partial \nu_E}}_E\mathrm ds\right)\label{eqn:jh_defn}
%
%
\end{align}
with the jumps $\jump{v_{\pw}}_{{E}}(z) $
%
for $z \in \mathcal{V}(E)$ and $E \in \mathcal{E}$ defined as follows. The edge-patch $\omega(E):=\text{\rm int}(T_+\cup T_-)$ of an interior edge 
$E=\partial T_+\cap\partial T_-\in\E(\Omega)$  is the interior of the union 
$T_+\cup T_-$ of two neighboring triangles $T_+$ and $T_-$. Fix the orientation of the unit normal $\nu_E$ along $E$ and label $T_{\pm}$ such that $\nu_{T_+}|_E=\nu_E=-\nu_{T_-}|_E$ is the outer normal of $T_+$ along $E$. Let $\partial_s$ denote the tangential derivative along an edge $E$.
Then the jump resp.\ average read $[v_{\rm pw}]_E:=(v_{\pw} |_{T_+} -v_{\pw} |_{T_-})$ resp.\ $\langle v_{\pw} \rangle_E\coloneqq\half\left(v_{\pw}|_{T_+}+v_{\pw}|_{T_-}\right)$ on $E \in \E(\Omega)$. 
For a boundary edge $E \subset\partial T\cap \partial\Omega$ contained in the unique triangle $T \in \T$, $v_E= v_T|_E$, set $\omega(E) ={\rm int}(T)$ and $\jump{ v_{\pw}}_{E} = v_{\pw}|_E $ resp.\ $\langle v_{\pw}\rangle_E:=v_{\pw}|_E$. Let $\tau_E$ denote the unit tangent of fixed orientation along an edge $E\in\E$ and abbreviate $h_{\E},\nu_{\E},\tau_{\E},$ resp.\ $\jump{v_\pw}_{\E}$ as functions on the skeleton $\bigcup \E$ with $h_{\E}|_E\coloneqq h_E, \nu_{\E}|_E\coloneqq\nu_E,\tau_{\E}|_E\coloneqq\tau_E,$ resp.\ $\jump{v_\pw}_{\E}|_E:=\jump{v_\pw}_E$ for any $E\in\E$.
The piecewise integral mean operator $\Pi_{\E,0}$ reads $\Pi_{\E,0}(v)|_E\coloneqq\Pi_{E,0}(v)\coloneqq\fint_E v \;\ds$ for any $v\in L^2(E)$ and $E\in\E$.
%
%

\medskip \noindent 
The remaining parts of this paper apply the abstract results from Section \ref{sec:Abstract a posteriori error control} to fourth-order problems with the Sobolev spaces $V=X=Y:=H^2_0(\Omega)$
endowed with the energy norm $\trb{\bullet}\equiv(\trb{\bullet}_\pw)|_V\equiv(\|\bullet\|_h)|_V$ for the seminorm $\trb{\bullet}_\pw\coloneqq(a_\pw(\bullet,\bullet))^{1/2}  $ in $H^2(\T)$
and the discrete spaces $V_h=X_h=Y_h \subseteq P_2(\T)$ equipped with the induced norm $\|\bullet\|_h$ of the common superspace $\widehat V=\widehat X=\widehat Y:=H^2(\T)$ given as
\begin{align}
    \label{hnorm}
\|v_{\pw}\|_{h}^2 &:= \trinl v_{\pw} \trinr_{\pw}^2 + j_h(v_{\pw}, v_{\pw}) \qquad\text{for all } v_{\pw} \in H^2(\cT).
\end{align}
The subsequent analysis also requires the Morley finite element space
\[
\cM(\cT):=\left\{ v_\cM\in P_2(\cT) \; \vrule\;
%
%
%
%
%
%
%
\jump{v_\M}_E(z) = 0\text{ and }\int_{E}\jump{\frac{\partial v_\cM}{\partial \nu_E}}_E{\ds}=0\text{ for all }E\in\E\text{ and } z\in\mathcal V(E)
%
\right\}
\]
that lies in the kernel of $j_h$, i.e., $j_h(v_\M,\bullet)=0$ such that $\|v_\M\|_h=\trb{v_\M}_\pw$ for all $v_\M\in\M(\T)$, and comes with 
the Morley interpolation operator $I_\M$ that generalizes from $V$ to $H^2(\T)$ by averaging~\cite{ccnnlower2022}.
%
\begin{defn}[{Morley interpolation~\cite[Definition 3.5]{ccnnlower2022}}]   \label{def:morleyii}
	Given any $v_{\pw} \in H^2(\cT)$, define $I_{\rm M}v_{\pw} := v_{\rm M} \in {\rm M}(\cT)$ by its degrees of freedom as follows.  For any interior vertex $z \in \mathcal{V}(\Omega)$ with the set of attached triangles $\cT(z)$ of cardinality $|\cT(z)| \in \mathbb{N}$ and for any interior edge {{$E \in \mathcal{E}(\Omega)$}},
%
	\begin{align}
	v_{\rm M}(z) := |\cT(z)|^{-1} \sum_{K \in \cT(z)} (v_{\pw}\vert_{K})(z)\;\;\text{ and } \fint_{E} \dfrac{\partial v_{\rm M}}{\partial \nu _{\rm E}}\,\mathrm{d}s := \fint_{E} \left\langle \dfrac{\partial v_{\rm pw}}{\partial \nu_{E}} \right\rangle_E\,\mathrm{d}s.
	\end{align} 
	The remaining degrees of freedom at the vertices and edges on the boundary are set zero owing to the homogeneous boundary conditions.
\end{defn}
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
\noindent
An important property \cite[Eqn.~(3.5)]{ccnnlower2022} of the generalized Morley interpolation is the $a_\pw$-orthogonality
\begin{equation} \label{eqn:rightinverse}
    a_{\pw}(v_2, v-I_{\M} v)  =0 \qquad\text{for all } v \in V \text{ and all } v_2 \in P_2(\T).
\end{equation}
The point is that there exists a right-inverse $J:\M(\T)\to V$ of $I_\M$, that is, $I_{\M}J v_\M= v_\M$ for all $v_\M \in \M(\T)$, as in \cite{DG_Morley_Eigen,ccnn2021}, \cite[Lemma 3.7, Theorem 4.5]{ccnnlower2022} with
$%
    \|v_h-JI_\M v_h\|_h\lesssim\min_{v\in V}\|v-v_h\|_h
$
for all $v_h\in P_2(\T)$
such that $P=Q=S\coloneqq JI_\M: V_h \rightarrow V$ and $R \in \{{\rm id}, I_\M, JI_\M \}$ satisfy the assumptions \eqref{quasioptimalsmootherP}--\eqref{quasioptimalsmootherS} of Section \ref{sec:Abstract a posteriori error control}.
%
%
The last ingredient is a bounded transfer operator  $I_h: \M(\T) \rightarrow V_h$ 
%
that 
%
is either 
%
%
the identity $I_h\coloneqq{\rm  id}$ for the Morley, dG, and WOPSIP schemes with $\M(\T)\subset V_h$ or
%
%
$I_h\coloneqq I_{\rm C}$ for C$^0$IP with $V_h:=S^2_0(\T)\coloneqq P_2(\T) \cap H^1_0(\Omega)$ defined, for all $v_\M\in \M(\T)$, by
\begin{align} \label{eq:ic}
(I_{\rm C} v_\M)(z)=
\begin{cases}
	v_\M(z) &\text{for all } z \in {\mathcal V},\\
	\langle{v_\M}\rangle_E (z)  &\text{for } z= \text{mid}(E), \; E \in \E(\Omega), \\
	0 &\text{for } z= \text{mid}(E), \; E \in \E(\partial \Omega).
\end{cases}
\end{align}
The boundedness of $I_h$ implies $\|I_h\|\coloneqq\sup_{v_\M\in\M(\T)}\|I_h v_\M\|_h/\trb{v_\M}_\pw<\infty$.
%
%
%
%
%
%
%
%
%
	%
%
		%
%
%
	%
%
%
		%
%
	%
%
 %
%
	%
%
%
%
%
%
%
%
%
%
%
\subsection{Explicit residual-based a posteriori estimator}\label{sub:explicit_aposteriori}
Any general source $F \in H^{-2}(\Omega)$ can be written with $L^2$ functions $f_0 \in L^2(\Omega), f_1 \in L^2(\Omega; {\mathbb R}^2), f_2 \in L^2(\Omega; {\mathbb S})$ \cite[Thm.~7.1]{CCBGNN22} as 
\begin{align} \label{eqn:newone}
F (\varphi) := \int_{\Omega} (f_0\; \varphi + f_1 \cdot \nabla \varphi + f_2 : D^2 \varphi) \dx \text{ for all } \varphi \in H^2_0(\Omega).
\end{align}
This definition extends to arguments $\varphi_\pw \in H^2(\T)$ by replacing $\varphi, \nabla \varphi, D^2 \varphi$ by their piecewise versions $\varphi_\pw, \nabla_\pw \varphi_\pw, D^2_\pw \varphi_\pw$. In the applications below, the approximation $v_h \in V_h \subset P_2(\T)$ is fixed 
 and $\Gamma_{\pw}(v_h,v_h,\bullet) \in H^{-2}(\Omega) $ has a structure as in \eqref{eqn:newone}, namely
\begin{align}\label{eqn:newtwo}
\Gamma_{\pw}(v_h,v_h, \varphi) = \int_{\Omega} (\Gamma_0\; \varphi + \Gamma_1 \cdot \nabla \varphi 
+ \Gamma_2: D^2 \varphi) \dx  \text{ for all } \varphi \in H^2_0(\Omega)
\end{align} 
for piecewise polynomials $\Gamma_0 \in P_k(\T)$, $\Gamma_1 \in P_k(\cT; {\mathbb R}^2), $
 $\Gamma_2 \in P_k(\cT; {\mathbb S})$ of degree at most $k\in\mathbb N_0$.
 The Lebesgue functions in \eqref{eqn:newone} and the polynomial degree $k\in\mathbb N_0$ give rise to oscillations 
 \begin{align} \label{eqn:newfour}
 {\rm osc}_k(F,\T) &:= \| h_\T^2(f_0-\Pi_k f_0)\|_{L^2(\Omega)} + \| h_\T(f_1-\Pi_k f_1)\|_{L^2(\Omega)} 
 + \| f_2-\Pi_k f_2\|_{L^2(\Omega)}.
 \end{align}
 %
 
\begin{example}[Navier-Stokes] \label{ex:3.1} The trilinear form $\Gamma_\pw$ for the Navier-Stokes equations in Section \ref{sec:nse} below is given by \eqref{eqn:newtwo} for $k=1$ with $\Gamma_1= \Delta_{\pw} v_h \: {\rm Curl}_{\pw} v_h$ and $\Gamma_0=0$, $\Gamma_2=0$.
\end{example}
\begin{example}[von K\'{a}rm\'{a}n]\label{ex:3.2}
For the von K\'{a}rm\'{a}n equiations in Section~\ref{sec:vke} and vector-valued approximation $\mathbf{v_h}\equiv\big(\vha,\vhb\big)\in V_h\times V_h$, 
 choose $\Gamma_0=[\vha,\vhb]$  resp.\  $\Gamma_0=-1/2[\vha,\vha]$ and $\Gamma_1= 0$, $\Gamma_2=0$ with the von K\'{a}rm\'{a}n  bracket 
$[\bullet,\bullet]$
defined in Subsection \ref{vke:model_intro} and $k=0$. 
%
\end{example}
%
 %
 %
 %
 %
 
 \medskip
\noindent Recall $\tau_{\E},\nu_{\E},[\bullet]_{\E}$, and the piecewise integral mean operator $\Pi_{\E,0}$ from Subsection \ref{sub:triangulation, interpolation, and smoother}. The error estimators $ \mu_1(\T) + \mu_2(\T) + \mu_3(\T)=: \mu(\T) $ and $\eta(\T)$ are defined in terms of 
\begin{equation}\label{eqn:lambdas}
\begin{array}{ll}
{\Lambda}_0:= \Pi_k f_0 - \Gamma_0 \in P_k(\T), \\
\Lambda_1:= \Pi_k f_1 - \Gamma_1 \in  P_k(\cT; {\mathbb R}^2),  \\  
\Lambda_2 := \Pi_k f_2 - D^2_{\pw} v_h - \Gamma_2 \in P_k(\cT; {\mathbb S})
\end{array}
\end{equation}
with $\vartheta=1$ for $I_h={\rm id}$ resp. $\vartheta=0$ for $I_h=I_{\rm C}$ by 
 \begin{align*}
 \mu_1(\T) &:= \big\| h_{\T}^2 (\Lambda_0 - {\rm div}_{\pw} \Lambda_1 +{\rm div}^2_{\pw} 
 \Lambda_2) \big\|_{L^2(\Omega)}, \\
%
%
%
 %
%
  \mu_2(\T) &:= \big\| h_{\E}^{3/2}\jump{\Lambda_1 - {\rm div}_{\pw} \: 
 \Lambda_2 - \partial_s (\Lambda_2 \tau_{\E})}_{\E} \cdot \nu_{\E}  \big\|_{L^2(\E(\Omega))},  \\
  \mu_3(\T) &:= 
 %
  \big\|h_{\E}^{1/2} (1-\vartheta \: \Pi_{{\E},0}) \jump{\Lambda_2 \nu_{\E}}_{\E} \cdot  \nu_{\E} \big\|_{L^2(\E(\Omega))}, 
  %
  %
  %
  %
%
 %
  %
  %
  %
  %
  %
\\
\eta(\T)&:=\| v_h-{JI_\M}  v_h\|_{h}.
 %
 %
 \end{align*}
 %
 %
%
 %
%
%
The following theorem controls the intermediate residual $\rho(M)$ from \eqref{a} with $M=\|I_h\|$ from the abstract reliability estimate \eqref{eqn:apost} by the explicit a posteriori error estimators $\mu(\T)$ and $\eta(\T)$. Define
\begin{align}\label{eqn:varrho}
    \rho\coloneqq
\sup_{\stackrel{y \in Y, \|y \|_Y = 1}{z:=y- J I_\M I_hI_\M y} } 
\big( F(z)-a( J I_\M v_h,z) -
\Gamma_{\pw}(Rv_h, Rv_h, z)  \big).
\end{align}


 \begin{theorem}[reliability and efficiency up to data oscillations] \label{thm:releff}
 Under the present notation $V=X=Y\equiv H^2_0(\Omega)$, the choices $P=Q=S=JI_\M$, and
 $R=\{{\rm id}, I_\M, J I_\M \}$, it holds 
 \begin{align*}
& (a)   \; \rho(\|I_h\|) \leq\rho\lesssim  \eta(\T) + \mu(\T) +{\rm osc}_k(F,\T), \\
&
 (b) \;  \eta(\T) + \mu(\T)\lesssim  \rho(0)+ {\rm osc}_k(F,\T), 
 \\
 & (c) \; \eta(\T) \approx \big\|h_{\E}^{1/2} \jump{D^2_\pw v_h}_{\E}\tau_{\E}\big\|_{L^2(\E)} + j_h(v_h,
		v_h)^{1/2}.
  \end{align*}
\end{theorem}
\noindent The estimate Theorem~\ref{thm:releff}.c is well-known from \cite[Theorem 5.6]{CCBGNN22}, \cite{DG_Morley_Eigen}. The remaining parts of this section therefore focus on the proofs of Theorem~\ref{thm:releff}.a and b.
%
\begin{rem}[role of \eqref{eqn:QO}] The a priori results in \cite{CCNNGRDS22} establish \eqref{eqn:QO} for  $S=Q=JI_\M$ in \eqref{eqn:discrete} and this leads to efficiency. Theorem \ref{thm:apost} is fairly general and the reliability estimate allows for $S \neq Q$; but then \eqref{eqn:QO} involves an additional additive term $\Gamma(Ru_h, Ru_h, (S-Q)y_h) = O(h_{\rm max}^{\alpha})$ \cite[Theorem 5.1]{CCNNGRDS22}. This extra term behaves like a given $L^2$ function (in terms of piecewise derivatives of $Ru_h$)  times the mesh-sizes up to some power  $\alpha \ge 0$. The application to Navier-Stokes leads to $\alpha=1$ and this is of the correct asymptotic rate (or even better), while the application to \vket ~even allows for $\alpha=2$ {\cite{CCNNGRDS22}}. However, this extra term is {\it not} a residual term (in general) and efficiency is left open as in \cite{CCGMNN_semilinear,kim_morley_2021}. 
The new schemes from \cite{CCNNGRDS22} with $P=Q=S=JI_\M$ in \eqref{eqn:discrete}  enable an efficient and reliable a posteriori error control in this paper for general sources.  
\end{rem}

\begin{comment}
{\begin{theorem} \cite{CCBGNN22} \label{thm:fromold}There exist positive constants $C_{\rm rel}^{\ell}, C_{\rm eff}^{{\ell}}$, that exclusively depend o the shape regularity of $\T$ and on the polynomial degree $k \in {\mathbb N}_0$ such that 
 $C_{\rm rel}^{\ell} \trinl \Lambda \circ (1-J_hI_h I_\M) \trinr_* \le \mu(\T) \le C_{\rm eff}^{{\ell}} \trinl \Lambda \trinr_*$.
 \end{theorem}
 \begin{lemma} \cite{CCBGNN22} \label{lem:newone} Any $v \in H^2_0(\Omega)$ satisfies $$ \sum_{j=0}^2 \|h_\T^{j-2} (v- JI_\M I_h I_\M v) \| \lesssim \mu(\T) \lesssim \trinl  \Lambda \trinr_*.$$
 \end{lemma}
 \begin{lemma} \cite{CCBGNN22} \label{lem:newtwo} $\trinl v_h- JI_\M v_h \trinr_{\pw} \approx \eta(\T) \lesssim \|v_h-Jv_h\|_h \lesssim \trinl u-v_h\trinr_{\pw}$.
 \end{lemma} }
 \footnote{to be checked and quoted properly}
\end{comment}
\subsection{Proof of Theorem~\ref{thm:releff}.a.} \label{appl:rel}
The definition of $\rho(M)$ for $M\coloneqq\|I_h\|$ in \eqref{a} implies $\rho(M)\leq\rho$.
Indeed, for any $v\in V$ with $\trb{v}=1$ and $v_h:= I_h I_\M v \in V_h$, it follows that $\|v_h\|_h \le \|I_h\| \trinl  I_\M v \trinr_{\pw} \le M$ from 
$ \trinl I_\M v\trinr_{\pw} \le \trinl v \trinr = 1$ and so $v_h\equiv I_hI_\M v$ is admissible (the last inequality is a consequence of the Pythogoras theorem and the orthogonality \eqref{eqn:rightinverse}). %
The reflexivity of $V \equiv H^2_0(\Omega)$ leads to $w \in V$ with $\trinl w \trinr = 1$ and
\begin{equation}\label{eqn:star1}
    \rho(\|I_h\|)  \leq \rho \le   F(z)-a(Pv_h,z)-\Gamma_{\pw}(Rv_h,Rv_h,z) 
\end{equation}
for $z:=w-JI_\M w_h$. 
%
%
Recall $\Lambda_0,\Lambda_1, \Lambda_2$ from \eqref{eqn:lambdas} and define $\Lambda \in H^{-2}(\Omega)$ by 
%
 \begin{equation} \label{eqn:newthree}
 \Lambda(\varphi)= \int_{\Omega} (\Lambda_0 \varphi + \Lambda_1 \cdot \nabla \varphi + \Lambda_2: D^2 \varphi) \dx \text{ for all } \varphi \in H^2_0(\Omega).
 \end{equation}
%
Observe carefully that the definition of $F$ in \eqref{eqn:newone} and $\Lambda$ in \eqref{eqn:newthree}  lead to 
\begin{align}\label{eqn:startwo}
F-a(Pv_h,\bullet)-\Gamma_{\pw}(Rv_h,Rv_h,\bullet) 
& = F- \Pi_k F + \Lambda + a_{\pw}(v_h-Pv_h,\bullet) \nonumber \\
& \quad  +  \Gamma_{\pw}(v_h,v_h,\bullet)-\Gamma_{\pw}(Rv_h,Rv_h,\bullet).
\end{align}
Here and throughout, $\Pi_k F \in H^2(\T)^*$ is defined by
\begin{align}\label{eqn:Pi_F_def}
    \Pi_k F (v_\pw) := 
\int_{\Omega} \big( v_\pw \Pi_k f_0 +
\nabla_{\pw}v_\pw \cdot \Pi_k f_1+ D^2_{\pw} v_{\pw}:
\Pi_k f_2 \big) \dx \quad\text{for } v_{\pw} \in H^2(\T).
\end{align}
The six terms on the right-hand side in \eqref{eqn:startwo} are controlled as follows. Since $z=(1-J I_\M I_h I_\M )w$ vanishes at the vertices for all $w \in V$, the stability result \cite[Lemma 5.1]{CCBGNN22} 
 \begin{align} \label{eqn:C_stability}
 \sum_{m=0}^2 |h_\T^{m-2} (1- JI_\M I_h I_\M )w |_{H^m(\T)} & \le C_{\rm stab} \trinl w  \trinr \text{ for all } w \in H^2_0(\Omega)
 \end{align}
controls the  data oscillation term  
\cite[Lemma 7.2]{CCBGNN22} by  
\begin{align} \label{eqn:fbound}
   (F- \Pi_k F)(z) &= \int_{\Omega} \Big( 
   (f_0- \Pi_k f_0) z + 
    (f_1- \Pi_k f_1) \cdot \nabla z +
   (f_2- \Pi_k f_2): D^2 z \Big) \dx \nonumber \\
   & 
    \le C_{\rm stab} {\rm osc}_k(F,\T) \trinl z \trinr. 
\end{align}
%

\medskip \noindent A Cauchy inequality, the boundedness of $\Gamma_{\rm pw}$, $\trinl v_h-Pv_h \trinr_{\pw} \leq \|v_h-Pv_h\|_h$ from \eqref{hnorm}, and the definition of $\eta(\T) $ %
 reveal 
    \begin{align}
    a_\pw(v_h-Pv_h,z) & \le  \trinl v_h-Pv_h \trinr_{\pw} 
    \trinl z \trinr \le \eta(\T) \trinl z \trinr, \\
    %
%
%
%
 \Gamma_{\pw}(v_h,v_h,z)-\Gamma_{\pw}(Rv_h,Rv_h,z)  & \le \|\Gamma_\pw\| (1+\|R\|) \|v_h\|_{h}
\|v_h-Rv_h\|_{h} \trinl z \trinr \nonumber \\
 &\le \|\Gamma_\pw\| (1+\|R\|)\lamr\big(\trb{u} +  \beta/ ((1+\Lambda_{\rm P}) \|\Gamma\|)\big)\; \eta(\T)  \trinl z \trinr\label{eqn:G_bound2a}
%
%
\end{align}
with the arguments from the analysis of $S_2$ in Subsection~\ref{S2}, 
$\trinl v_h-Rv_h \trinr_{\pw} \leq \|v_h-Rv_h\|_h$ from \eqref{hnorm}, \eqref{quasioptimalsmootherP}, \eqref{quasioptimalsmootherR}, and \eqref{eqn:vhbound}  in the last step.
It remains to control $\Lambda$,   where we employ results from the linear situation. 
The appendix of the preliminary work on linear problems \cite{CCBGNN22} provides the estimate 
\begin{align} \label{eqn:starfour}
\trinl \Lambda \circ (1-JI_\M I_h I_\M) \trinr_* \le 
C_{\rm rel}^{\rm lin} \: \mu(\T).
 \end{align}
 Since $z \equiv w- JI_\M I_h I_\M w$ acts as a test function in \eqref{eqn:starfour} and $\trb{w}=1$, we infer 
 \begin{align} \label{eqn:lam}
 \Lambda(z) \leq\trinl \Lambda \circ (1-JI_\M I_h I_\M) \trinr_* \trb{w}\le C_{\rm rel}^{\rm lin}\: \mu(\T).
 \end{align}
   Since $\trinl z \trinr \le C_{\rm stab}$ from \eqref{eqn:C_stability},
   %
   the reliability  $\rho(\|I_h\|) \leq\rho\lesssim  \eta(\T) + \mu(\T) +{\rm osc}_k(F,\T)$ follows from \eqref{eqn:startwo},\eqref{eqn:fbound}--\eqref{eqn:G_bound2a}, and \eqref{eqn:lam} in \eqref{eqn:star1}. 
   The above constants $C_{\rm stab}$ and $C_{\rm rel}^{\rm lin} $ exclusively depend on the shape regularity of the triangulation $\T$ and the polynomial degree $k$ of the $\Lambda_0,\Lambda_1,\Lambda_2$ in \eqref{eqn:newtwo}. 
   %
   \qed
\begin{comment}
Given $M=\|I_h\|$ and $y \in H^2_0(\Omega)$ with $\trinl y \trinr =1$, let $y_h= I_h I_\M y \in V_h$ and observe $\|y_h\|_h \le \|I_h\| \trinl  I_\M y \trinr_{\pw} \le \|I_h\|=M$.
 Hence 
 \begin{align} \label{eqn:newfour1}
 \rho(\|I_h\|) & \le \trinl  F-a(Pv_h,\bullet)-\Gamma_{\pw}(Rv_h,Rv_h,\bullet) \circ 
 (1 - JI_\M I_h I_\M)\trinr_* \nonumber \\
 & \quad + C_7 (\trinl  a_{\pw}(Pv_h-v_h,\bullet)  \trinr_*+ \trinl \Gamma_{\pw}(v_h,v_h,\bullet)-\Gamma_{\pw}(Rv_h,Rv_h,\bullet) \trinr_*  )
 \end{align}
 from triangle inequalities and for $C_7=\| 1-JI_\M I_h I_\M\|_{L(V_h, H^2_0(\Omega))}$.
 The last two terms in \eqref{eqn:newfour1} are controlled with Lemma~\ref{lem:newone} and Lemma~\ref{lem:newtwo} as
 \begin{align}
 \trinl a_{\pw}(v_h-Pv_h,\bullet)  \trinr_* & \le  \trinl v_h - Pv_h \trinr_{\widehat{X}} = \trinl v_h-JI_\M v_h\trinr_{\pw} \lesssim  C_8 \eta(\T)  \label{eqn:apw} \\
  \trinl \Gamma_{\pw}(v_h,v_h,\bullet)-\Gamma_{\pw}(Rv_h,Rv_h,\bullet) \trinr_* & =\trinl \Gamma_{\pw}(v_h-Rv_h,v_h,\bullet)+\Gamma_{\pw}(Rv_h,v_h-Rv_h,\bullet) \trinr_* 
   \le{C_9  \eta(\T)} \label{eqn:g}%
  %
 \end{align}
with the boundedness of $a_{\pw}$, $\Gamma_{\pw}$, \eqref{eqn:PR}, and \eqref{eqn:vhbound},   in the second step above and for the constant $C_9:=  \|\Gamma\| (2+\Lambda_{\rm R})(1+\|R\|) \|v_h\|_{X_h}$, that also depends on $\|v_h\|_h$.
%

\noindent The definition of $\Lambda$ in \eqref{eqn:newthree} leads in the first term of the upper bound in \eqref{eqn:newfour} to 
\begin{align}\label{eqn:newseven}
\trinl  F-a(Pv_h,\bullet)-\Gamma_{\pw}(Rv_h,Rv_h,\bullet) \circ 
 (1 - JI_\M I_h I_\M)\trinr_* & \le \trinl  \Lambda  \circ 
 (1 - JI_\M I_h I_\M)\trinr_*\nonumber \\
 & \qquad + \trinl  (F-\Pi_k F) \circ 
 (1 - JI_\M I_h I_\M)\trinr_*
\end{align}
for the functional $\Pi_k F$ defined by \eqref{eqn:newone} with $f_0,f_1,f_2$ replaced by
$\Pi_k f_0,\Pi_k f_1,\Pi_k f_2$. The first term on the right- hand side of \eqref{eqn:newseven} is equivalent to $\mu(\T)$ owing to Theorem \ref{thm:fromold}, while the second term reads
\begin{align}\label{eqn:neweight}
& \trinl F-\Pi_k F\trinr_* = \sup_{\trinl v \trinr \le 1} \int_{\Omega} ((f_0- \Pi_k f_0) (v-\Pi_k v) + (f_1- \Pi_k f_1). \nabla (v-\Pi_k v) + (f_2- \Pi_k f_2) : D^2v) \dx  \nonumber\\
& \quad \lesssim \|h_\T^2 (f_0-\Pi_k f_0)\|_{L^2(\Omega)} +\|h_\T (f_1-\Pi_k f_1)\|_{L^2(\Omega)}+
\|f_2-\Pi_k f_2\|_{L^2(\Omega)}= {\rm osc(F)}
\end{align}
with $(F-\Pi_k F)  \perp P_k(\T)$ in the first step and Lemma~\ref{lem:newone} in the last step.
The summary of the above estimate reads
$$ \rho(\|I_h\|) \le C_{\rm rel} (\eta(\T) + \mu(\T) + {\rm osc(F)}). \qed$$
\end{comment}
%
\subsection{Proof of Theorem~\ref{thm:releff}.b} 
The efficiency $\eta(\T) \equiv \|v_h-Pv_h\|_h \le \Lambda_{\rm P }\| u-v_h \|_{h} $ follows from \eqref{quasioptimalsmootherP} for $P\equiv JI_\M$ as in \cite[Thm~5.6]{CCBGNN22}.%

\medskip \noindent The efficiency of $\mu(\T) \le  C_{\rm eff}^{\rm lin}
\trinl \Lambda \trinr_*$ is established in \cite[Theorem A.1]{CCBGNN22}  with $C_{\rm eff}^{\rm lin}$ that exclusively depends on the shape-regularity of $\T$. The definitions of $\Lambda= \Pi_k F - a(v_h,\bullet ) - \Gamma_{\pw} (v_h,v_h,\bullet)$ and $\rho(0)$ therefore lead to 
%
\begin{align} \label{eqn:mubound}
\mu&(\T)  \le C_{\rm eff}^{\rm lin} \trinl \Lambda \trinr_*  \le  \trinl \Pi_k F-a(v_h,\bullet)-\Gamma_{\pw}(v_h,v_h,\bullet) \trinr_* \nonumber \\
&\le  \rho(0) + \trinl F- \Pi_k F\trinr_* + \trinl a_{\pw} (v_h - Pv_h,\bullet) \trinr_* 
  + \trinl \Gamma_{\pw}(v_h,v_h,\bullet)-\Gamma_{\pw}(Rv_h,Rv_h,\bullet) \trinr_*.
%
\end{align}
%
%
 %
  %
   %
    %
%
%
%
%
%
%
%
%
%
%
%
A Cauchy inequality and the boundedness and $\Gamma_{\pw}$ provide, for any $z\in V$, that
  \begin{align} \label{bounda}
    a_\pw(v_h-Pv_h,z) & \le \trb{ v_h-Pv_h }_\pw\trb{z}
    \le \Lambda_{\rm P} \|u-v_h\|_{h}\trinl z \trinr,  \\ 
 \Gamma_{\pw}(v_h,v_h,z)\!-\!\Gamma_{\pw}(Rv_h,Rv_h,z)  & \le \|\Gamma_\pw\| (1\!+\!\|R\|) \|v_h\|_{h}
\|v_h-Rv_h\|_{h} \trinl z \trinr \nonumber \\
 &\le \|\Gamma_\pw\| (1\!+\!\|R\|)\lamr\big(\trb{u} \!+ \! \beta/ ((1\!+\!\Lambda_{\rm P}) \|\Gamma\|)\big) 
\|u\!-\!v_h\|_{h} \trinl z \trinr \label{eqn:bound_gamma}
\end{align}
with $\trinl v_h-Pv_h \trinr_{\pw} \leq \|v_h-Pv_h\|_h$ from \eqref{hnorm}, \eqref{quasioptimalsmootherP} for  \eqref{bounda} and $\trinl v_h-Rv_h \trinr_{\pw} \leq \|v_h-Rv_h\|_h$ from \eqref{hnorm}, \eqref{quasioptimalsmootherR},  and \eqref{eqn:vhbound} in the last step. 
%
The combination of \eqref{eqn:mubound}--\eqref{eqn:bound_gamma} and \eqref{eqn:fbound}
lead to 
%
$\mu(\T) \lesssim \rho(0) + {\rm osc}_k(F,\T) + \|u-v_h \|_h$ and conclude the proof.
%
\qed
%
 %
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%

%

%


\section{Application to Navier-Stokes equations} \label{sec:nse}
%
\subsection{Stream-function vorticity formulation of Navier-Stokes equations} \label{sec:prob}
The stream-function vorticity formulation of the incompressible 2D Navier--Stokes problem for a given load $F\in H^{-2}(\Omega)$ in a polygonal domain $\O \subset \R^2$ seeks $u \in V:=H^2_0(\O) (\equiv X\equiv Y)$  such that%
\begin{equation} \label{NS_eqa}
 \Delta^2u + \frac{\partial}{\partial x}\Big((-\Delta u)\frac{\partial u}{\partial y}\Big)- \frac{\partial}{\partial y}\Big((-\Delta u)\frac{\partial u}{\partial x}\Big)= F \quad\text{ in } \O.
\end{equation}
(The bi-Laplacian $\Delta^2$ reads $\Delta^2\phi:=\phi_{xxxx}+\phi_{yyyy}+2\phi_{xxyy}$.)  The analysis of extreme viscosities lies beyond the scope of this article, and so the viscosity of the
 bi-Laplacian in \eqref{NS_eqa} is set one. 
 Recall the semi-scalar product $a_{\rm pw}:H^2(\T)\times H^2(\T)\to\mathbb R$ and the induced piecewise $H^2$ seminorm $\trinl \bullet \trinr_{\rm pw} $ that is a norm \cite{ccnn2021} on $V+\M(\cT) \subset H^2(\T)$ from Subsection \ref{sub:triangulation, interpolation, and smoother}.
 Define the bounded trilinear form $\Gamma_{\pw}(\bullet,\bullet,\bullet)$ by 
\begin{align} \label{deftns:bilinear}
%
\Gamma_{\pw}(\widehat{\eta}, \widehat{\chi},\widehat{\phi}) :=\sum_{T\in\T}\int_{T}^{} \Delta \widehat{\eta}\,\Big(\frac{\partial \widehat{\chi}}{\partial y}\frac{\partial \widehat{\phi}}{\partial x}-\frac{\partial \widehat{\chi}}{\partial x}\frac{\partial \widehat{\phi}}{\partial y}\Big) \dx\qquad\text{for all }\widehat{\eta},\widehat{\chi},\widehat{\phi} \in   H^2(\T).
\end{align} 
%
%
Given $a:=a_{\pw}|_{V \times V}$ and $\Gamma:=\Gamma_{\pw}|_{V\times V \times V}$, 
%
%
the weak formulation of  \eqref{NS_eqa} seeks $u \in V$ such that
\begin{align} \label{NS_weak}
a(u,w) + \Gamma(u,u,w) = F(w)\fl w \in V.
\end{align}
Given any $F\in V^*\equiv H^{-2}(\Omega)$, there exist solutions to \eqref{NS_weak}, which are possibly singular but carry elliptic regularity. 
In the case of small loads ($\trb{F}_*\|\Gamma\|<1$), the weak solution is unique and a regular root, cf.~\cite[Chap.~IV.§2--3]{GR:FiniteElementMethods1986} and \cite{NS_FE79,Tem:NavierStokesEquations1995} for proofs.
%
The a posteriori error analysis below concerns some approximation $v_h \in  V_h$  to a regular root  ${u} \in V$ of the continuous problem~\eqref{NS_weak}.}
\subsection{Five quadratic discretizations}\label{sec:discrete_schemes}
This subsection presents the {Morley},  two variants of {dG},  ${ C^0}$IP, and  WOPSIP discretizations for \eqref{NS_weak}.
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
 %
%
%
%
%
%
%
%
%
The discrete space $V_h\equiv X_h\equiv Y_h$ becomes $V_h\coloneqq\M(\T)$  for Morley, $V_h\coloneqq P_2(\T)$ for dG and WOPSIP schemes, and $V_h\coloneqq S^2_0(\cT)\coloneqq P_2(\cT) \cap H^1_0(\Omega)$ for the  $C^0$IP scheme. For all  $v_{\rm pw}, w_{\rm pw} \in H^2(\cT)$ and  parameters $\sigma_1,\sigma_2, \sigma_{\ip}>0$ sufficiently large (but fixed in applications) to guarantee the stability of $a_h$ below, the method-dependent penalty forms $c_{\dg}, c_{\rm P}$, and $c_{\rm IP}$ read
\begin{align}\label{eqn:cdG_def}
    c_{\rm dG}(v_{\pw}, w_{\pw})&\coloneqq \sum_{E\in\cE}\bigg(\frac{\sigma_1}{h_E^3}\int_E \jump{v_{\rm pw}}_E \jump{w_{\rm pw}}_E\ds+ \frac{\sigma_2}{h_E}\int_E\jump{ \frac{\partial v_{\rm pw}}{\partial  \nu_E}}_E  \jump{\frac{\partial w_{\rm pw}}{\partial  \nu_E}}_E \ds\bigg),\\
    c_{\rm P}(v_{\pw}, w_{\pw})&\coloneqq \sum_{E \in \mathcal{E}} 
h_{E}^{-4} \bigg(\sum_{z \in \mathcal{V}(E)} \Big(\jump{v_{\rm pw}}_E   
\jump{w_{\rm pw}}_E\Big)(z)+\int_E\jump{ \frac{\partial v_{\rm pw}}{\partial  \nu_E}}_E  \ds \int_E\jump{\frac{\partial w_{\rm pw}}{\partial  \nu_E}}_E \ds\bigg),\label{eqn:c_P_def}
\end{align}
and $c_{\rm IP}\coloneqq c_{\rm dG}|_{(V+S^2_0(\T))\times (V+S^2_0(\T))}$ with $\sigma_{\rm IP}\coloneqq \sigma_{2}$. Define the discrete bilinear forms 
\[a_h:= a_{\rm pw} + {\mathsf b}_h+ 
{\mathsf c}_h:\left(V + V_h\right)\times \left(V + V_h\right)\to \mathbb R, \] with $a_{\pw}$ from \eqref{deftns:bilinear} for the Morley, dG I, ${ C^0}$IP, and  WOPSIP discretizations and $a_{\pw}$ replaced by $(\Delta_{\pw} \bullet, \Delta_{\pw} \bullet)_{L^2(\Omega)}$
%
%
for the dG II scheme, and  ${\mathsf b}_h$ and ${\mathsf c}_h $ from Table \ref{tab:spaces} for some $-1\leq\theta\leq 1$.
%
%
%
%
%
%
%
%
The method-dependent norms induced by $a_\pw+c_h$ for dG I, WOPSIP, and $C^0$IP {(resp.  
$(\Delta_\pw\bullet,\Delta_\pw\bullet)_{L^2(\O)} +c_h$ for dG II as in \cite{SM:HpversionInteriorPenalty2007})
are, except for WOPSIP, equivalent to the universal norm $\|\bullet \|_{h}$ from 
\eqref{hnorm}. Notice that $\|\bullet\|_h=\trb{\bullet}_\pw$ in $V+\M(\T)$ follows from \eqref{hnorm}.
\begin{lemma}[{Equivalence of norms \cite[Thm.~4.1]{ccnngal}}] \label{lem:equivalence}
	It holds 
 %
 $\| \bullet \|_{h} \approx \|\bullet \|_{\rm dG}\equiv \big(\trinl \bullet \trinr_{\rm pw}^2 +c_{\dg}(\bullet,\bullet)\big)^{1/2}$ on $V + P_2(\cT)$ and $\| \bullet \|_{h} \approx \|\bullet \|_{\rm IP}\equiv \big(\trinl \bullet \trinr_{\rm pw}^2 +c_{\rm IP}(\bullet,\bullet)\big)^{1/2}$ on $V + S^2_0(\cT)$. \qed
\end{lemma}  
In contrast to this, the WOPSIP norm $\|\bullet \|_{\rm P} \equiv \big(\trinl \bullet \trinr_{\rm pw}^2 +c_{\rm P}(\bullet,\bullet)\big)^{1/2}$ involves smaller powers of the mesh-size and is (strictly) stronger than $\|\bullet\|_h$, i.e., $h_T\leq h_{\rm max}$ implies
\begin{align}\label{eqn:P_norm}
    j_h\leq h_{\rm max}^2 c_{\rm P}\qquad\text{and}\qquad \|\bullet\|_h\leq (1+h_{\rm max}^2)^{1/2}\|\bullet\|_{\rm P}.
\end{align}
%
%
%
%
%
%
%
%
%
%
%
%
%
%
\noindent  The applications in this paper consider the choice $P\equiv Q\equiv S\equiv JI_\M$  %
that allows the first reliable and efficient a posteriori error estimate for the stream-function vorticity formulation of the Navier-Stokes equations. 
%
%
%
%
%
\begin{table}[]
\centering {\footnotesize
\begin{tabular}{|c|c|c|c|c|c|}
\hline
Scheme & Morley & \multicolumn{1}{c|} {dG I} &  $C^0$IP & WOPSIP & dG II \\ \hline
%
%
%
%
%
%

%

%

%

%
%
%



%

$\mathcal{J}(\bullet ,\bullet)  $ & -- & \multicolumn{2}{c|}{{${{{}\displaystyle \sum_{E\in\cE}\int_E \langle D^2v_2\;\nu_E\rangle_E} \cdot \jump{\nabla w_2}_E\ds}$}}  & -- &${{{}\displaystyle \sum_{E\in\cE}\int_E \jump{\frac{\partial v_2}{\partial \nu_E}}_E\langle \Delta_{\pw}w_2\rangle_E} }\,\ds$   \\\hline


${\mathsf b}_h(\bullet,\bullet)$ & 0 &
\multicolumn{2}{c|}{\begin{minipage}{3.6cm}
\centering
\vspace{3pt}
$ -\theta \mathcal{J}(v_2,w_2) {- \mathcal{J}(w_2,v_2)} $
%
\end{minipage}}
& 0 & $-\theta \mathcal{J}(v_2,w_2) {- \mathcal{J}(w_2,v_2)}$  \\ \hline
${\mathsf c}_h(\bullet,\bullet)$ & 0 &
$ c_\dg(\bullet,\bullet)$ & $ c_{\rm IP}(\bullet,\bullet)$ &$ c_{\rm P}(\bullet,\bullet)$ &$ c_\dg(\bullet,\bullet)$ \\\hline
%
$I_{h}$ & ${\rm id}$ & \multicolumn{1}{c|}{${\rm id}$} & $I_{\rm C}$  from \eqref{eq:ic} & ${\rm id}$ & ${\rm id}$ \\ \hline  
\end{tabular}
%
\caption{Bilinear forms with $\theta\in[-1,1]$ and operator $I_h$ in Section \ref{sec:nse}. }
\label{tab:spaces}}
\end{table}
%
%
%
		%
%
%
%
%
%
  %
	%
		%
	%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
Recall $\tau_{\E},\nu_{\E},[\bullet]_{\E}$, and the piecewise integral mean operator $\Pi_{\E,0}$ from Subsection~\ref{sub:triangulation, interpolation, and smoother} and abbreviate $\mathrm{Curl}\coloneqq(\partial/\partial y; - \partial/\partial x)$.
Given $\vartheta=1$ for $I_h={\rm id}$ resp. 
$\vartheta=0$ for $I_h=I_{\rm C}$, the local error estimators on $T\in\T$,
 \begin{align*}
 \sigma^2(T) & := |T|^2 \|\Pi_k f_0-  {\rm div}_{\pw} (\Pi_k f_1) +{\rm div}^2_{\pw}  (\Pi_k f_2) \|^2_{L^2(T)} \\
& \quad + |T|^{3/2} \|\jump{\Pi_k f_1 -\Delta v_h \: {\rm Curl} v_h -  {\rm div} (\Pi_k f_2) -
\partial_s ( \Pi_k f_2) \tau_{\E}}_{\E}  \cdot \nu_{\E} \|^2_{L^2(\partial T \setminus \partial \Omega)}\\
& \quad + |T|^{1/2}  { \| (1-\vartheta\Pi_{\E,0}) \jump{(\Pi_k f_2-  D^2 v_h)\nu_{\E}}_{\E} \cdot  \nu_{\E} \|_{L^2(\partial T \setminus \partial \Omega)}^2} 
\\
&\quad+|T|^{1/2} \big\|[D^2v_h]_{\E}\tau_{\E}\big\|_{L^2(\partial T)}^2+\sum_{E \in \mathcal{E}(T)} \Big(\big| \Pi_{E,0} \jump{\partial_\nu v_h}_E \big|^2 + |T|^{-1}\hspace{-0.6em} \sum_{z \in \mathcal{V}(E)} \big|\jump{v_h}_E(z)\big|^2 \Big)
%
%
%
     \end{align*}
define the a posteriori error estimator $\sigma(\T) := \sqrt{\sum_{T \in \T} \sigma^2(T)}$ by the $\ell^2$ sum convention.
\begin{rem}[Classical case]
    The a posteriori error analysis in \cite{CCGMNN_semilinear,kim_morley_2021} for the classical situation $R=S=Q={\rm id}$ and $F\equiv f\in L^2(\Omega)$ suffers from unclear efficiency.
\end{rem}
\begin{theorem}[A posteriori error control] \label{thm:apost_ns_final}
Given a regular root $u \in V$ to \eqref{NS_weak} with $F\in H^{-2}(\Omega)$ and $k\in {\mathbb N}$, there exist $\varepsilon, \delta,\varrho 
>0$ such that the following holds for any $\displaystyle\cT\in\bT(\delta)$ and $P\equiv Q\equiv S\equiv JI_\M$.
$(a)$ There exists a unique discrete solution $u_h\in V_h$ to \eqref{eqn:discrete} for the Morley, dG I \& II, and $C^0$IP scheme in Table~\ref{tab:spaces} with $\|  u-u_h\|_{h} \le\varepsilon$ and any $v_h \in V_h$ with $\|u_h-v_h\|_h \le \varrho$ satisfies
$$\| u-v_h \|_{h}  + {\rm osc}_k(F,\T) \approx \sigma(\T)  + \|u_h-v_h\|_{h} + {\rm osc}_k(F,\T).$$
$(b)$ For the WOPSIP scheme in Table~\ref{tab:spaces}, there exists a unique discrete solution $u_h\in V_h$ to \eqref{eqn:discrete} with $\| u-u_h\|_{h} \le\varepsilon$ and any $v_h \in V_h$ with $\|u_h-v_h\|_h \le \varrho$ satisfies
\begin{align}\label{eqn:WOPSIP_NVS_a}
    \| u-v_h \|_{h}  +\|u_h-v_h\|_{h} +  {\rm osc}_k(F,\T) &\approx \sigma(\T)  + \|u_h-v_h\|_{h} + {\rm osc}_k(F,\T),\\
    \| u-v_h \|_{\rm P}+\|u_h-v_h\|_{h}  +{\rm osc}_k(F,\T) &\approx \sigma(\T)  +c_{\rm P}(v_h,v_h)^{1/2}+ \|u_h-v_h\|_{h} + {\rm osc}_k(F,\T).\label{eqn:WOPSIP_NVS_b}
\end{align}
\end{theorem}
\noindent The Morley, dG I \& II, and $C^0$IP schemes satisfy the discrete consistency \eqref{eqn:H} and quasi-optimality \eqref{eqn:QO} so that the proof of Theorem \ref{thm:apost_ns_final} is already prepared in Theorems \ref{thm:apost} and \ref{thm:releff}.
The proof for the WOPSIP method (without \eqref{eqn:H} and \eqref{eqn:QO}) requires modifications in Subsection~\ref{sub:WOPSIP_NSV} below.
\begin{proof}[Proof of Theorem \ref{thm:apost_ns_final}.a]
The a priori analysis \cite[Thm.~8.1]{CCNNGRDS22} verifies the quasi-optimality \eqref{eqn:QO} and provides universal constants $\varepsilon_0,\delta_0>0$ that guarantee, for any $\T\in\TT{\delta_0}$, the unique existence of a discrete solution $u_h\in V_h$ to \eqref{eqn:discrete} with $\|u-u_h\|_h\leq \varepsilon_0$. 
A density argument for $\varepsilon\coloneqq\min\{\varepsilon_0,\beta/\left(3(1+\LP)\|\Gamma\|\right)\} $ leads to $\delta\leq\delta_0$ such that $\|u-u_h\|_h<\varepsilon$ for any $\T\in\TT\delta$.
This reveals \eqref{eqn:QO} and {\bf(L1)--(L3)} for $\delta,\varepsilon,\kappa\coloneqq2/3$, and $\varrho\coloneqq\beta/\left(3(1+\LP)\|\Gamma\|\right)$.
The abstract a posteriori error control from 
Theorem~\ref{thm:apost} applies with the abstract a posteriori error control of $\|u-v_h\|_h$ in terms of $\rho(\|I_h\|), \|(1-JI_\M)v_h\|_h$, and the efficient algebraic error $\|u_h-v_h\|_h$.
Section \ref{subsection:new} applied to $\Gamma_\pw$ from \eqref{deftns:bilinear} leads to 
${\Lambda}_0:= \Pi_k f_0, \; \Lambda_1:= \Pi_k f_1 -  \Delta_{\pw} v_h \: {\rm Curl}_{\pw} v_h, \; 
\Lambda_2 := \Pi_k f_2 - D^2_{\pw} v_h$ in \eqref{eqn:lambdas}.
Theorem~\ref{thm:releff}.a controls $\rho(\|I_h\|)+\|(1-JI_\M)v_h\|_h$ with the a posteriori term $\mu(\T) +\eta(\T)$, that is efficient by Theorem~\ref{thm:releff}.b and Theorem~\ref{thm:apost}.b, plus data oscillations ${\rm osc}_k(F,\T)$. The equivalence $\mu(\T) +\eta(\T)\approx \sigma(\T)$ follows with $h_E\approx h_T\approx |T|^{1/2}$ from shape-regularity and Theorem~\ref{thm:releff}.c. This concludes the proof.
%
%
%
    %
%
%
%
%
 %
  %
%
\end{proof}
\subsection{Modifications for WOPSIP}\label{sub:WOPSIP_NSV}


There are two reasons why the weakly over-penalized symmetric
interior penalty (WOPSIP) scheme from \cite{BrenGudiSung10} requires little modifications in the above analysis.
The first is the failure of \eqref{eqn:H} and (somehow related) the failure of \eqref{eqn:QO} in the stated  form. The second is that the natural
WOPSIP norm $\|\bullet\|_{\rm P}$ from \eqref{eqn:P_norm} is very strong and \eqref{eqn:WOPSIP_NVS_a}
states the error estimate in the (partly) weaker norm $\|\bullet\|_h$.

\medskip 
\noindent 
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
The starting point for the analysis in this subsection is a modified version of \eqref{eqn:H} already applied in the analysis of linear problems \cite[Thm.~6.9]{CCBGNN22} that follows from $j_h(v_{\pw}, w_{\M})=0=c_{\rm P}(v_{\pw}, w_{\M})$ for all $(v_{\pw},v_{\M})\in H^2(\T)\times \M(\T)$.
Recall that $\|J\|$ abbreviates the operator norm of
$J: \M(\T)\to V$ when $\M(\T)$ and $V$ are endowed with the norm $\trinl \bullet \trinr_{\rm pw}\equiv\|\bullet\|_h|_{V+\M(\T)}$ and $a_h = a_{\rm pw} + {c}_{\rm P}$ for WOPSIP. %
\begin{lemma}[modified \eqref{eqn:H}] \label{lem:H_WOPSIP}
   Any  $(v_2,w_\M)\in P_2(\T)\times \M(\T)$ satisfies
\begin{align}\label{eqn:H_WOPSIP}
    a( J I_{\M} v_2, J w_{\M})- a_h(v_2,w_{\M})\le \| J \|
\trinl v_2- JI_\M v_2\trinr_{\pw} \trinl w_{\M} \trinr_{\pw}.
\end{align}
\end{lemma}
\begin{proof} For the WOPSIP scheme,  ${ c}_{\rm P}(v_2, w_\M) = 0$  for $(v_{2},v_{\M})\in P_2(\T)\times \M(\T)$ shows
	\begin{align*} %
a(JI_\M v_2, Jw_\M)	- a_{h}(v_2, w_\M)  &= 
a(JI_\M v_2, Jw_\M)-a_{\rm pw}(v_2, w_\M) \\
&=a_{\pw}(JI_\M v_2-v_2, Jw_\M) \le \|J\| 
\trinl v_2- JI_\M v_2\trinr_{\pw} \trinl w_{\M} \trinr_{\pw}
	\end{align*}
 with $a_{\rm pw}(v_2, w_\M- Jw_\M)=0 $ from \eqref{eqn:rightinverse} and the boundedness of $a_{\rm pw}(\bullet,\bullet)$ in the last line above.
\end{proof}
\noindent A careful revisit of the arguments in Section \ref{sec:Abstract a posteriori error control} with \eqref{eqn:H_WOPSIP} instead of \eqref{eqn:H} reveals a modified reliabiltiy
\begin{align}\label{eqn:reliability_WOPSIP}
    \| u- v_h\|_{h}  \lesssim \varrho  + \|(1-JI_\M)v_h\|_{h} +\|u_h-v_h\|_{h} %
\end{align}
with $\rho$ from \eqref{eqn:varrho} instead of $\rho(M)$ in Theorem \ref{thm:apost}. Theorem \ref{thm:apost_ns_final} can follow with Theorem \ref{thm:releff}.
%
%
%
\begin{proof}[Proof of Theorem \ref{thm:apost_ns_final}.b]
The a priori results for WOPSIP \cite[Thm.~8.13]{CCNNGRDS22} reveal the convergence under uniform mesh refinement in the norm $\|\bullet\|_{\rm P}$ and provide universal constants $\varepsilon_0,\delta_0>0$ such that, for any $\T\in\TT{\delta_0}$, a unique discrete solution $u_h\in V_h$ to \eqref{eqn:discrete} exists with $\|u-u_h\|_{\rm P}\leq \varepsilon_0$.
Since $\|\bullet\|_{\rm P}$ is stronger than $\|\bullet\|_h$ by \eqref{eqn:P_norm}, the convergence also follows in the weaker norm $\|\bullet\|_h$ and $h_{\rm max}\leq \delta_0$ implies the unique existence of a discrete solution $u_h\in V_h$ to \eqref{eqn:discrete} with $\|u-u_h\|_h\leq(1+\delta_0^2)^{1/2}\epsilon_0$. 
A density argument for $\varepsilon\coloneqq\min\{(1+\delta_0^2)^{1/2}\varepsilon_0,\beta/\left(3(1+\LP)\|\Gamma\|\right)\} $ leads to $\delta\leq\delta_0$ such that $\|u-u_h\|_h<\varepsilon$ for any $\T\in\TT\delta$.
This implies {\bf(L1)--(L3)} in the weaker norm $\|\bullet\|_h$ for $\delta,\varepsilon,\kappa\coloneqq2/3$, and $\varrho\coloneqq\beta/\left(3(1+\LP)\|\Gamma\|\right)$.
Hence, the setting of Section \ref{sec:Abstract a posteriori error control} applies and the proofs in Subsection~\ref{sec:apost} follow verbatim for $u_h,v_h \in V_h$, and $u \in V $ until \eqref{eqn:u-vh} that becomes
\begin{align} \label{eqn:triangle}
    \|u-v_h\|_{h} & \le 
     \|v_h -J I_\M v_h\|_{h}+
    \beta^{-1} (1-\kappa)^{-1} \|N(J I_\M v_h)\|_{V^*}
 \end{align}
 in the current setting.
The subsequent estimation of $\|N(J I_\M v_h)\|_{V^*}$ involves the split
%
$N(J I_\M v_h; y)=S_1+S_2+S_3$ as in \eqref{eqn:newb} for any $y \in Y \equiv H^2_0(\Omega)$ with $\trb{y}=1$ and the particular choice $y_h\coloneqq I_\M y\in \M(\T)$ in the definition of $S_1, S_3$ (instead of any $y_h\in P_2(\T)$ in Subsection~\ref{sub:varrho}).
The point of this modification is twofold. 
First, the supremum over $y\in Y$ with $w:=y- J I_\M y_h= y- J I_\M y \in V$ reveals
\begin{align}
    S_1:=a(J I_\M v_h,w) + \Gamma_{\pw}(Rv_h,Rv_h, w) -{F}(w) \le \rho.
\end{align}
Second, Lemma \ref{lem:H_WOPSIP} with $y_h\equiv I_\M y\in \M(\T)$ and $\trb{\bullet}_\pw\leq\|\bullet\|_h$ from \eqref{hnorm} result in \eqref{eqn:H_application} for $\Lambda_{\rm C}\coloneqq \|J\|$ without the need of \eqref{eqn:H}.
With this alternate derivation of \eqref{eqn:H_application}, the control of 
\begin{align}
    S_2&\coloneqq \Gamma_{\pw}(JI_\M v_h,JI_\M v_h,y) -\Gamma_{\pw}(JI_\M v_h,JI_\M v_h, y)\lesssim \|v_h -J I_\M v_h\|_{h},\\
    S_3&\coloneqq a(JI_\M v_h,JI_\M y)-F(JI_\M y) + \Gamma_{\pw}(Rv_h,Rv_h, JI_\M y)\lesssim \|v_h -J I_\M v_h\|_{h}+\|u_h-v_h\|_{h}\label{eqn:S3_bound_WOPSIP}
\end{align} %
follows verbatim from Subsection \ref{S2}--\ref{ssub:abstract_reliability_final} with $\|y_h\|_{h} = \trinl I_\M y\trinr_{\rm pw} \le \trinl y \trinr=1 \equiv M$.
This and \eqref{eqn:triangle}--\eqref{eqn:S3_bound_WOPSIP} verify the alternate reliability estimate \eqref{eqn:reliability_WOPSIP}. 
Theorem~\ref{thm:releff} further controls $\rho, \|(1-JI_\M)v_h\|_h$ in terms of the explicit a posteriori error terms $\mu(\T) +\eta(\T)\approx \sigma(\T)$  plus data oscillations ${\rm osc}_k(F,\T)$.
The efficiency of $\sigma(\T)$ with respect to $\|u-u_h\|_h$ plus data oscillations follows from Theorems~\ref{thm:releff}.b and~\ref{thm:apost}.b. This verifies \eqref{eqn:WOPSIP_NVS_a}. The sum of \eqref{eqn:WOPSIP_NVS_a} and $c_{\rm P}(v_h,v_h)=c_{\rm P}(u-v_h,u-v_h)$ with 
$ \|\bullet\|_h^2+c_{\rm P}=\trb{\bullet}^2+j_h+c_{\rm P}\approx \|\bullet\|_{\rm P}^2$
from \eqref{eqn:P_norm} reveal \eqref{eqn:WOPSIP_NVS_b} and conclude the proof.
\begin{comment}
and 
The point of this modification is that in the estimation of 
selects some $y_h:= I_\M y \in \M(\T)$ to attain the infimum in $\varrho(M)$ from \eqref{eqn:varrho}.
as a Morley function with $\|y_h\|_{\rm P} = \trinl I_\M y\trinr_{\rm pw} \le \trinl y \trinr=1 =:M.$ Then the split $N(J I_\M v_h; y) =S_1+S_2+S_3$ from \eqref{eqn:newb}
provides for $w:=y- J I_\M y_h= y- J I_\M y \in V$
$$S_1:=a(J I_\M v_h,w) + \Gamma_{\pw}(Rv_h,Rv_h, w) -{F}(w) \le \varrho:=
\sup_{\stackrel{y \in Y, \|y \|_Y = 1}{z:=y- J I_\M y} } 
\Big( F(z)-a( J I_\M v_h,z) -
\Gamma_{\pw}(Rv_h, Rv_h, z)  \Big).$$
The control of $\varrho$ (instead of $\varrho(M)$) follows verbatim as Subsection~\ref{appl:rel} and provides $\varrho \lesssim \eta(\T)+\mu(\T) +{\rm osc}_k(F,\T)$. The control of \eqref{t2} in Subsection~\ref{S2} allows the norm $\|\bullet\|_h$ (rather than $\|\bullet \|_{\rm P}$) and provides as in the case of dG that 
\[ S_2 \lesssim \|v_h\|_h \|v_h- J I_\M v_h \|_h.\]
The analysis of $S_3$ is crucial and the first two terms in the right-hand side of \eqref{eqn:s3} read
\begin{align}\label{new:s3}
    a(J I_\M v_h, J I_\M y)- a_{\rm P}(v_h,I_\M y )  \le \|J\| \trinl v_2- J I_\M v_2 \trinr_{\rm pw} 
\end{align}
with Lemma~\ref{modifiedlemma} and $\trinl I_\M y \trinr_{\pw} \le 1$ in the last step. The third term in the right-hand side of \eqref{eqn:s3} reads
\[ a_h(v_h-u_h,I_\M y)= a_{\pw}(v_h-u_h,I_\M y) \le \trinl v_h-u_h \trinr_{\pw}.\]
The arguments in \eqref{eqn:t2a} apply to the norm $\| \bullet \|_h$ (instead of $\|\bullet\|_{\rm P}$) and provide the upper bound  
$\lesssim \|u_h-v_h\|_h$ (as for the dG schemes) for the $\|\bullet\|_h$ norm. The summary reads $$S_3 \lesssim  \trinl v_2- J I_\M v_2 \trinr_{\rm pw}  +\|u_h-v_h\|_h$$
and is sharper in each of the two terms than expected from the WOPSIP norms. In fact, the WOPSIP norm $\|\bullet \|_{\rm P}$ only arises from the choice \eqref{eqn:triangle} and provides 
\[  \|u-v_h\|_{\rm P}  \le 
     \|v_h -J I_\M v_h\|_{\rm P}+ \|u_h-v_h\|_h+ \eta(\T)+\mu(\T) +{\rm osc}_k(F,\T).\]
  \noindent The split in the weaker norm $\|\bullet \|_h$ in \eqref{eqn:triangle} provides
  \[  \|u-v_h\|_{h}  \le 
     \|v_h -J I_\M v_h\|_{h}+ \|u_h-v_h\|_h+ \eta(\T)+\mu(\T) +{\rm osc}_k(F,\T).\]
This clarifies the reliability and efficiency follows from $\varrho \le \varrho(0) \lesssim \|u-v_h\|_h$. The efficiency analysis of the remaining terms follow as for the dG and so ---
\footnote{I am not sure as to what we do more to complete- don't we  need efficiency of $\|v_h -J I_\M v_h\|_{\rm P}$? }
\end{comment}
\end{proof}
%
%
%
%
%
%
%
%
%
%
%
%

%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%

%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%

%
%
%
%
%
%
%
%
%
%
%
%





%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
\section{Application to von K\'{a}rm\'{a}n equations }\label{sec:vke}
The von K\'{a}rm\'{a}n equations model a nonlinear plate \cite{CiarletPlates,Ciarlet2013} in two coupled PDE and require the product spaces
$X=Y=\bv := V \times V$ of $V\equiv H^2_0(\Omega)$
%
%
%
%
%
with norm  $\trinl\bullet\trinr$  
%
defined by $\trinl\boldsymbol\varphi\trinr:=(\trinl \varphi_1 \trinr^2+\trinl \varphi_2\trinr^2)^{1/2}$ for all $\boldsymbol\varphi=(\varphi_1,\varphi_2)\in \bv$. 
%
%
%
\subsection{Von K\'{a}rm\'{a}n equations}
\label{vke:model_intro}
%
Given any load $F\in H^{-2}(\Omega)$, the \vket~seek a solution ${\bf u} \equiv  ( \ua, \ub) \in  \bV $\;%
to
\begin{align}
\Delta^2 \ua =[\ua,\ub]+ F \;\;\text{ and }\;\;\Delta^2 \ub =-\half[\ua,\ua] 
%
\label{vkedGb}
%
\end{align}
in a bounded polygonal Lipschitz domain $\Omega \subset \mathbb{R}^2$.
Here and throughout this section, the (symmetric) von K\'{a}rm\'{a}n bracket $[\bullet,\bullet]$ reads $[\eta,\chi]:=\eta_{xx}\chi_{yy}+\eta_{yy}\chi_{xx}-2\eta_{xy}\chi_{xy}$.
%
%
%
%
%
 Recall the bilinear form ${a}_{\rm pw}$ and $\widehat V\equiv H^2(\T)$ from Subsection \ref{sub:triangulation, interpolation, and smoother}. %
 Let $\widehat{\bv}\coloneqq\widehat V\times \widehat V$ and define the trilinear forms $\Gamma_{\pw, 1}, \Gamma_{\pw, 2}:\widehat V\times \widehat V\times \widehat V$ and $\mathbf{\Gamma}_\pw:\widehat{\bv}\times \widehat{\bv}\times \widehat{\bv}$  by %
 \begin{align*}
     \Gamma_{\pw, 1}(\widehat{\xi},\widehat{\theta},\widehat{\varphi})&:=
-\sum_{T\in\T}\int_T [\widehat{\xi},\widehat{\theta}]\,\widehat{\varphi}\dx,\qquad%
\Gamma_{\pw, 2}(\widehat{\xi},\widehat{\theta},\widehat{\varphi}):=
\half\sum_{T\in\T}\int_T [\widehat{\xi},\widehat{\theta}]\,\widehat{\varphi}\dx,\\
\mathbf{\Gamma}_\pw(\widehat{\boldsymbol\xi },\widehat{\boldsymbol\theta},\widehat{\boldsymbol\varphi}) &:=\Gamma_{\pw,1}(\widehat{\xi_1},\widehat{\theta_2},\widehat{\varphi}_1)+\Gamma_{\pw,2}(\widehat{\xi_1},\widehat{\theta_1},\widehat{\varphi}_2)
 \end{align*}
for all $\widehat{\xi},\widehat{\theta},\widehat{\varphi} \in  \widehat V$ and $\widehat{\boldsymbol\xi }=(\widehat{\xi_1},\widehat{\xi_2}),\widehat{\boldsymbol\theta}=(\widehat{\theta_1},\widehat{\theta_2}),\widehat{\boldsymbol\varphi}=(\widehat{\varphi}_1,\widehat{\varphi}_2)\in \widehat{\bv}$.
%
%
Given $\displaystyle  a:= {a}_{\pw}|_{V \times V},$ %
$\Gamma_1:=\Gamma_{\pw,1}|_{V \times V\times V}$, and $\Gamma_2:=\Gamma_{\pw,2}|_{V \times V\times V}$, the weak formulation of~\eqref{vkedGb} seeks  ${\bf u} \equiv  ( \ua, \ub) \in  \bV $ with
\begin{align} \label{vk_weak}
a(\ua,\varphi)+ \Gamma_1(\ua,\ub,\varphi) = F(\varphi) \quad\text{and}\quad
a(\ub,\varphi) + \Gamma_2(\ua,\ua,\varphi)   = 0\quad\text{for all }\varphi\in V.       
%
%
\end{align} 
%
 %
%
%

\medskip \noindent   For all $\boldsymbol\theta=(\theta_1,\theta_2)$ and $\boldsymbol\varphi=(\varphi_1,\varphi_2)\in  \bv$, define %
%
$${\boldsymbol a}(\boldsymbol\theta,\boldsymbol\varphi) :={} a(\theta_1,\varphi_1) + a(\theta_2,\varphi_2),\quad\text{and}\quad\mathbf F(\boldsymbol\varphi) \coloneqq F(\varphi_{1})
%
%
.$$ 
Given $\mathbf{\Gamma}\coloneqq \mathbf{\Gamma}_\pw|_{V\times V\times V}$, the vectorised formulation of~\eqref{vk_weak} seeks ${\bf u}=(\ua,\ub)\in \bv$ such that
\begin{equation}\label{VKE_weak}
\mathbf N({\bf u};\boldsymbol\varphi):={\boldsymbol a}({\bf u},\boldsymbol\varphi)+\mathbf \Gamma({\bf u},{\bf u},\boldsymbol\varphi)- \mathbf{F}(\boldsymbol\varphi)=0\fl \boldsymbol\varphi \in \bv.
\end{equation}
Given any $F\in V^*\equiv H^{-2}(\Omega)$, there exist solutions to \eqref{vk_weak}, which are possibly singular but carry elliptic regularity; the weak solution is unique and a regular root in the case of small loads, cf.~\cite{MN:ConformingFiniteElement2016,Ciarlet2013,Kni:ExistenceTheoremKarman1967} for proofs. The a posteriori error analysis below concerns some approximation ${\bf v}_{h}\in \bV_h \coloneqq  V_h\times V_h$  to a regular root  ${\bf u} \in \bV$ of the continuous problem~\eqref{vk_weak}.
%
}
%
%
%
%
%
%
\subsection{A posteriori error control for five quadratic discretizations} \label{sec:vke_disc}
This subsection applies the abstract a posteriori error analysis from Section \ref{subsection:new}--\ref{sec:nse} to the Morley, dGI\&II, $C^0$IP, and WOPSIP schemes for~\eqref{VKE_weak}.
Recall the discrete space $ V_h$ from Subsection~\ref{sec:discrete_schemes} together with the bilinear forms $\mathsf{b}_h$ and $\mathsf{c}_h$
%
from Table \ref{tab:spaces} for the five methods.
%
%
%
For any $\boldsymbol\theta_h\equiv(\theta_{h,1},\theta_{h,2}),\boldsymbol\varphi_h\equiv(\varphi_{h,1},\varphi_{h,2})\in X_h\equiv Y_h\equiv\bv_h\equiv V_h\times V_h$, the discrete bilinear form ${\boldsymbol a}_h : \bv_h \times \bv_h \rightarrow \mathbb{R}$ reads
\begin{equation}\label{eqn:apw_vke}
    \begin{aligned}
         {\boldsymbol a}_{h}(\boldsymbol\theta_h,\boldsymbol\varphi_h)
:={}& a_{\rm pw}(\theta_{h,1},\varphi_{h,1})+ \mathsf{b}_h(\theta_{h,1},\varphi_{h,1}) +  \mathsf{c}_h(\theta_{h,1},\varphi_{h,1})  \\
&+ a_{\rm pw}(\theta_{h,2},\varphi_{h,2}) +  \mathsf{b}_h(\theta_{h,2},\varphi_{h,2}) + \mathsf{c}_h(\theta_{h,2},\varphi_{h,2}).
    \end{aligned}
\end{equation}
The second dG scheme replaces $a_{\rm pw}$ by $(\Delta_{\pw} \bullet, \Delta_{\pw} \bullet)_{L^2(\Omega)}$.
%
%
%
%
%
%
%
%
%
%
Let  $\boldsymbol{R} \in \{\mathbf{id}, \boldsymbol{I}_{\rm M}, \boldsymbol{JI}_{\rm M} \}$ and $\boldsymbol{P}\equiv\boldsymbol Q\equiv\boldsymbol S \equiv\boldsymbol J\boldsymbol I_\M$ denote the vectorized versions of the respective operators from Subsection \ref{sub:triangulation, interpolation, and smoother} that apply componentwise.
The discrete scheme for~\eqref{VKE_weak} 
 seeks a solution ${\bf u}_{h}\in \bV_h$ to
\begin{align}\label{eqn:gen_scheme_vke}
\hspace{-0.7cm}\boldsymbol{N}_h({\bf u}_h;\Phi_h) := \boldsymbol a_{h}({\bf u}_{h},\boldsymbol\varphi_h)
+\mathbf\Gamma_{\pw}(\boldsymbol {R}{\bf u}_{h},\boldsymbol{R}{\bf u}_{h},
\boldsymbol{S}\boldsymbol\varphi_h)-\mathbf F( \boldsymbol{ Q}{\boldsymbol\varphi}_{h})=0 \fl \boldsymbol\varphi_h \in  \bv_h.
\end{align}
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
\begin{comment}
\begin{table}[H]
	\centering
	\begin{tabular}{|c|c|c|c|c|c|}
		\hline
		Scheme     & Morley & dG I       & $C^0$IP     & WOPSIP & dG II \\ \hline
		%
		$X_h = Y_h = \bV_h$          &  $\mathbf{M}(\cT)$      & $\boldsymbol{P}_2(\cT)$      & $\boldsymbol{S}^2_0(\cT)$ & $\boldsymbol{P}_2(\cT)$  & $\boldsymbol{P}_2(\cT)$      \\ \hline
		\begin{minipage}{2cm}
			\centering
			$\widehat{X} = \widehat{Y} = \widehat{\bV}  =\bV + \bV_h$
		\end{minipage}   &   $\bV + \mathbf{M}(\cT)$     & $ \bV + \Stb$          & $ \bV + \boldsymbol{S}^2_0(\cT)$  & $ \bV +  \Stb$   &  $ \bV + \Stb$     \\ \hline
		$\|\bullet \|_{\widehat{X}}$            & $\trinl \bullet \trinr_{\rm pw}$     & $\| \bullet \|_{\rm dG}$       &    $\| \bullet \|_{\rm IP}$  &  $\| \bullet \|_{\rm P}$ &$\| \bullet \|_{\rm dG}$      \\ \hline
%
%
		$I_{h}$ & ${\mathbf {id}}$ & ${\mathbf {id}}$ &$\boldsymbol{I}_{\rm C}$  & ${\mathbf  {id}}$ & ${\mathbf {id}}$ \\ \hline 
			$I_{X_h}=I_{\bV_h} = I_{h}\boldsymbol{I}_{\rm M}$           &  $\boldsymbol{I}_{\rm M}$ & $\boldsymbol{I}_{\rm M}$ & $\boldsymbol{I}_{\rm C}\boldsymbol{I}_{\rm M}$ & $\boldsymbol{I}_{\rm M}$ &  $\boldsymbol{I}_{\rm M}$    \\ \hline
%
%
%
%
%
%
	\end{tabular}
	\caption{Spaces, operators, and norms in Section \ref{sec:vke}.}
	\label{tab:spaces_vke}
\end{table}
\end{comment}
%
Recall $\tau_{\E},\nu_{\E},[\bullet]_{\E}$, and the piecewise integral mean operator $\Pi_{\E,0}$ from Subsection~\ref{sub:triangulation, interpolation, and smoother}. 
Set $\vartheta=1$ for Morley, dG I\& II, WOPSIP, and
$\vartheta=0$ for C$^0$IP.
The a posteriori error estimator $\boldsymbol{\sigma}(\T) := \sqrt{\sum_{T \in \T} \boldsymbol{\sigma}^2(T)}$ for some approximation ${\bf v}_h= (\vha,\vhb)\in \bV_h$  to a regular root  ${\bf u} \in \bV$ of the continuous problem \eqref{vkedGb} has on $T\in\T$ the contribution
\begin{equation*}%
    \begin{aligned}
\boldsymbol{\sigma}^2(T)& := |T|^2 \Big( \|\Pi_k f_0+[\vha,\vhb] - {\rm div}_{\pw} (\Pi_k f_1) +{\rm div}^2_{\pw}  (\Pi_k f_2) \|^2_{L^2(T)} + \|[\vha,\vha] \|^2_{L^2(T)} \Big) \\
& \quad + |T|^{3/2} \|\jump{\Pi_k f_1 - {\rm div} (\Pi_k f_2) -
\partial_s ( \Pi_k f_2) \tau_{\E}}  \cdot \nu_{\E} \|^2_{L^2(\partial T \setminus \partial \Omega)}\\
& \quad + |T|^{1/2} \Big( \big\|[D^2\vha]_{\E}\tau_{\E}\big\|_{L^2(\partial T)}^2+ { \big\| (1-\vartheta\Pi_{\E,0}) \big[\big(\Pi_k f_2-  D^2 \vha\big)\nu_{\E}\big]_{\E} \cdot  \nu_{\E} \big\|_{L^2(\partial T \setminus \partial \Omega)}^2}
\\
%
%
%
 %
& \quad \phantom{|T|^{1/2} \Big(}  +   \big\|[D^2\vhb]_{\E}\tau_{\E}\big\|_{L^2(\partial T)}^2+ { \big\| (1-\vartheta\Pi_{\E,0}) \big[{\big( D^2 \vhb\big)\nu_{\E}}\big]_{\E} \cdot  \nu_{\E} \big\|_{L^2(\partial T \setminus \partial \Omega)}^2} \Big)
\\
& \quad + \sum_{\ell=1,2} \sum_{E \in \mathcal{E}(T)} \Big(\big| \Pi_{E,0} \big[\partial_\nu \vhl\big]_E \big|^2 + |T|^{-1}\hspace{-0.6em} \sum_{z \in \mathcal{V}(E)} \big|\big[\vhl]\big]_E(z)\big|^2 \Big).  
    \end{aligned}
\end{equation*}
%
%
Abbreviate $\mathbf{c}_{\rm P}({\bf v}_h,{\bf v}_h)\coloneqq c_{\rm P}(\vha,\vha)+c_{\rm P}(\vhb,\vhb)$ with the WOPSIP penalty form $c_{\rm P}$ from \eqref{eqn:c_P_def}.%
\begin{theorem}[a posteriori error control]%
\label{thm:apost_vke_final}
Given a regular root ${\bf u} \in \bV$  to \eqref{VKE_weak} with $F\in H^{-2}(\Omega)$ and $k\in\mathbb N_0$, there exist $\varepsilon, \delta,\varrho 
>0$ such that \eqref{eqn:gen_scheme_vke} has a unique discrete solution ${\bf u}_h\in \bV_h$ to \eqref{eqn:gen_scheme_vke} with $\|  {\bf u}-{\bf u}_h\|_{h} \le\varepsilon$ for any $\displaystyle\cT\in\bT(\delta)$ and the following holds for $F$ given as in \eqref{eqn:newone}.
$(a)$ For the Morley, dG I \& II, and $C^0$IP scheme and $\boldsymbol{P}\equiv \boldsymbol {Q} \equiv \boldsymbol{S}\equiv \boldsymbol {J} \boldsymbol{ I}_\M$, any ${\bf v}_h \in \bV_h$ with $\|{\bf u}_h-{\bf v}_h\|_h \le \varrho$ satisfies
$$\| {\bf u}-{\bf v}_h \|_{h}  + {\rm osc}_k(F,\T) \approx\boldsymbol{\sigma}(\T)  + \|{\bf u}_h-{\bf v}_h\|_{h} + {\rm osc}_k(F,\T).$$
$(b)$ For the WOPSIP scheme and $\boldsymbol{P}\equiv \boldsymbol {Q} \equiv \boldsymbol{S}\equiv \boldsymbol {J} \boldsymbol{ I}_\M$, any ${\bf v}_h \in \bV_h$ with $\|{\bf u}_h-{\bf v}_h\|_h \le \varrho$ satifsies
\begin{align*}%
\| {\bf u}-{\bf v}_h \|_{h}  + \|{\bf u}_h-{\bf v}_h\|_h + {\rm osc}_k(F,\T) &\approx\boldsymbol{\sigma}(\T)  + \|{\bf u}_h-{\bf v}_h\|_{h} + {\rm osc}_k(F,\T),\\
\| {\bf u}-{\bf v}_h \|_{\rm P}  + \|{\bf u}_h-{\bf v}_h\|_h + {\rm osc}_k(F,\T) &\approx\boldsymbol{\sigma}(\T) + \mathbf{c}_{\rm P}({\bf v}_h,{\bf v}_h)^{1/2} + \|{\bf u}_h-{\bf v}_h\|_{h} + {\rm osc}_k(F,\T).
   %
\end{align*}
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
\end{theorem}
\begin{proof}
The proof employs the a priori analysis in \cite[Sec.~9]{CCNNGRDS22} for the existence of a local unique discrete solution and follows the lines of that of Theorem \ref{thm:apost_ns_final} for all the components behind the vector notation of this section. Indeed,
Theorem \ref{thm:apost}.a and Theorem \ref{thm:releff}.a provide $\| {\bf u}-{\bf v}_h \|_{h}\lesssim \boldsymbol{\varrho}+\|{\bf v}_h-\boldsymbol{JI}_\M{\bf v}_h\|_h+ \|{\bf u}_h-{\bf v}_h\|_{h}$, where $\boldsymbol{\rho}\equiv \rho_1+\rho_2$ from \eqref{eqn:varrho} splits into the components
\begin{align}
        \rho_1&\coloneqq
\sup_{\stackrel{y \in Y, \|y \|_Y = 1}{z:=y- J I_\M I_hI_\M y} } 
\big( F(z)-a( J I_\M \vha,z) -
\Gamma_{\pw,1}(R\vha, R\vhb, z)  \big),\label{eqn:varrho_1}\\
        \rho_2&\coloneqq
\sup_{\stackrel{y \in Y, \|y \|_Y = 1}{z:=y- J I_\M I_hI_\M y} } 
\big(-a( J I_\M \vhb,z) -
\Gamma_{\pw,2}(R\vha, R\vha, z)  \big).\label{eqn:varrho_2}
\end{align}
The control of $\rho_1,\rho_2$ as in Theorem \ref{thm:releff} amounts in a large number of terms gathered together in the estimator $\boldsymbol{\sigma}(\T)$. As there is no additional mathematical difficulty, the further details are omitted.
%
%
%
%
 %
%
  %
%
%
%
 %
%
%
%
%
%
%
%
%
%
\end{proof}
\subsection{Single force} 
\label{sub:Single_forces}
Practical plate problems also concern line loads and single forces as discussed in \cite{CCBGNN22} for the linear biharmonic plate.
There are two amazing observations regarding a single force $\lambda_{\zeta} \pl$ with strength $\lambda_{\zeta} \in {\mathbb R}$ and the Dirac delta distribution $\pl \in H^{-2}(\Omega)$ at a finite set $A\subset \Omega$ of points $\zeta \in A$. 
First, single loads $\lambda_{\zeta} \pl$ decouple in the a posteriori error analysis %
from a general source $F \in H^{-2}(\Omega)$ given~by
\begin{align}\label{eqn:F_extended}
    F (\varphi) := \int_{\Omega} (f_0\; \varphi + f_1 \cdot \nabla \varphi + f_2 : D^2 \varphi) \dx + \sum_{\zeta\in A}\lambda_{\zeta} \pl(\varphi)\quad \text{for all } \varphi \in H^2_0(\Omega).
\end{align}
 in terms of 
 Lebesgue functions $f_0 \in L^2(\Omega), f_1 \in L^2(\Omega; {\mathbb R}^2), f_2 \in L^2(\Omega; {\mathbb S})$ as in \eqref{eqn:newone}.
 Second, a point load at an interior vertex $\zeta \in {\mathcal V}(\Omega)$ leads to a load in the discrete problem \eqref{eqn:discrete} but has no contribution to the a posteriori error estimate because the test functions for $F$ in $\rho_1$ from \eqref{eqn:varrho_1} vanish at all vertices $\mathcal V$.
 This has already been observed in \cite{ccnn2021, CCBGNN22} for linear problems. 
 Hence we consider a finite family $(\lambda_\zeta\pl: \zeta\in A)$ of single forces at $A\subset\Omega, |A|<\infty$ and distinguish $A\cap\mathcal V$ with no contributions $\mu(\zeta)=0$ and $A\setminus\mathcal V$ with a contribution $\mu(\zeta)$ to the a posteriori error control as follows.
 
\begin{comment}
 %
This subsection focuses on one single force $F=\lambda \pl$ with strength $\lambda \in {\mathbb R}$ and the Dirac delta distribution $\pl \in H^{-2}(\Omega)$ at a point $\zeta \in \Omega$. There are two amazing observations. First, the term $\lambda \pl$ (even a finite sum of those) decouples from $F= \lambda \pl+G\in H^{-2}(\Omega)$ with $G$ given in \eqref{eqn:newone} into  Lebesgue functions $f_0,f_1,f_2$ and hence all those functions are set zero in this subsection.
%
 Second, for a vertex $\zeta \in {\mathcal V}(\Omega)$, the functional $\pl$ applies to a test function $z= w - JI_\M I_h I_\M w$ that vanishes at ${\mathcal V} $ and so $\lambda(\pl )(z)= \lambda \: z(\zeta) =0$. Hence there remains no extra contribution in the a posteriori error estimate. In other words, $\zeta \in {\mathcal V}(\Omega)$ leads to a load in the discrete problem \eqref{eqn:discrete} but is not visible in the error estimate; this is already observed for linear problems in \cite{ccnn2021, CCBGNN22}. 
    
\end{comment}
\newcommand{\etaz}{\mu(\zeta)}
 \medskip \noindent
 Consider a single force $\lambda_\zeta\pl $ at a generic position $\zeta \in \Omega \setminus {\mathcal V}$ that is different from a vertex of the triangulation so that at most two triangles $T \in {\mathcal T}(\zeta):= \{ K \in \T: \zeta \in K\}$ contain $\zeta \in T$.
 Let  $h_\zeta\coloneqq\min {\{ }|T|^{1/2}: T \in \T(\zeta) {\}}, \omega(\zeta)\coloneqq\mathrm{int}(\cup \T(\zeta))$ and suppose the separation assumption
 \begin{align}\label{eqn:single_load_assumption}
     {\rm dist}(\zeta, {\mathcal V}) \gtrsim h_\zeta\quad\text{and}\quad |A\cap\omega(\zeta)|=1
     %
     \qquad\text{for all }\zeta\in A\setminus\mathcal V.
 \end{align}
 The following result extends Theorem \ref{thm:apost_vke_final} to right-hand sides with single forces at $A$.
 Define the novel estimator $\etaz\coloneqq|\lambda_\zeta| h_\zeta$ for a single load at $\zeta\in A$ and set $\mu(\mathcal M)\coloneqq\sum_{\zeta\in \mathcal M}\etaz$ for all $\mathcal M\subset A$.
%
 \begin{theorem}[single forces]\label{thm:apost_vke_dirac}
     Under the assumptions of Theorem \ref{thm:apost_vke_final}.a for $F\in H^{-2}(\Omega)$ given in \eqref{eqn:F_extended} for single forces at a finite set $A\subset\Omega$ with \eqref{eqn:single_load_assumption}, the Morley, dG I \& II, and $C^0$IP scheme satisfy
     $$\| {\bf u}-{\bf v}_h \|_{h}  + {\rm osc}_k(F,\T) \approx\boldsymbol{\sigma}(\T) + \mu(A\setminus\mathcal V) + \|{\bf u}_h-{\bf v}_h\|_{h} + {\rm osc}_k(F,\T).$$
     An analog to Theorem~\ref{thm:apost_vke_final}.b holds for the WOPSIP scheme where $\mu(A\setminus\mathcal V)$ is added on the respective right-hand sides.
 \end{theorem}
 
%
\begin{example}\label{ex:separation_condition}
    This separation condition \eqref{eqn:single_load_assumption} is met in the numerical benchmark in Subsection~\ref{sub:Numerical results for the Von Karman equation} for the centroid $\zeta=(-1/6;-1/6)$ of the L-shaped domain $\Omega$ that lies on an edge $E=\mathrm{conv}\{A,B\}\in\E$ parallel to the main diagonal for all triangulations (occuring from newest-vertex bisections) with $\zeta=1/3A+2/3B$ and ${\rm dist}(\zeta, {\mathcal V}) = h_E/3\geq \sqrt2h_\zeta/3 $ for the right-isosceles triangles in Subsection~\ref{sub:Numerical results for the Von Karman equation}.
\end{example}
\begin{proof}[Proof of Theorem \ref{thm:apost_vke_dirac}] The modifications to the source $F$ only enter the estimation of the term $\rho_1$ from \eqref{eqn:varrho_1} in Theorem \ref{thm:apost_vke_final}.
The reliability follows 
from Section~\ref{subsection:new} plus the analysis, for $\zeta\in A$, of the extra terms 
\[ |\lambda_{\zeta} \delta_{\zeta} (z)| \equiv |\lambda_{\zeta} z(\zeta)| \le \begin{cases}
    |\lambda_{\zeta}|\,C_{\rm BH}h_\zeta   |z|_{H^2(T)}&\text{if }\in A\setminus\mathcal V,\\
    0&\text{if }\in A\cap \mathcal V
\end{cases} \]
for any $z\coloneqq w-JI_\M I_hI_\M w$ with $w\in V$.
Indeed, $z$ vanishes at ${\mathcal V}$ and a Bramble-Hilbert lemma scales the Sobolev embedding $H^2(T_{\rm ref}) \hookrightarrow C(T_{\rm ref})$ from a reference triangle $T_{\rm ref}$ to $T$ with a constant $C_{\rm BH}$ that exclusively depends on the shape-regularity of $T$. Recall \eqref{eqn:C_stability} for $\trinl z \trinr \le C_{\rm stab} \trinl w \trinr$ and $\trinl w \trinr =1$ to deduce 
$\lambda_{\zeta} \delta_{\zeta} (z) \le C_{\rm BH} C_{\rm stab} \,\mu(\{\zeta\}\setminus \mathcal V)$
and involve this estimate in Subsection~\ref{appl:rel}. This outlines the proof of $\rho_1 \lesssim \boldsymbol{\sigma}(\T) + \mu(A\setminus\mathcal V) + {\rm osc}_k(F,\T)$;
the remaining details are straightforward from Theorem \ref{thm:apost_vke_final} and hence omitted. The efficiency of the additional a posteriori error terms $\mu(\zeta)$ for any $\zeta\in A\setminus\mathcal V$ requires the design of a test function $\psi \in V$ with a list of properties: 
\begin{equation}\label{eqn:psi_def}
    \begin{aligned}
        & \psi(\zeta)=1, \; \psi=0 \text{ at } {\mathcal V}, \;
{\rm supp}\: \psi \subseteq \overline{\omega(\zeta)}, \;
\psi|_T \perp P_k(T) \text{ in } L^2(T) \text{ for any triangle }
T \in \T,
%
\\
&  \; \psi|_E \perp P_k(E) \text{ in } L^2(E), 
\text{ and }
\nabla \psi|_E  \perp (P_k(E))^2 \text{ in } L^2(E)^2 \text{ along any edge } E \in \E.
    \end{aligned}
\end{equation}
This function can always be constructed and Supplement B provides an elementary design of $\psi$ in terms of Jacobi polynomials if $\zeta\in E\in\E$. An important detail is the scaling $\trinl \psi \trinr \approx h_{\zeta}^{-1}$ that requires the separation condition ${\rm dist}(\zeta, {\mathcal V}) \gtrsim h_\zeta $, while
 the universal case with $\zeta\in\Omega$ arbitrary involves a more refined analysis with a weight that is left for future research.
%
Recall $\Pi_kF$ from \eqref{eqn:Pi_F_def} and consider $\Lambda\coloneqq \Pi_kF-a_\pw(\vha,\bullet)-\Gamma_{\pw, 1}(\vha,\vhb, \bullet)$ as in
\eqref{eqn:newthree} with 
 \begin{align*}
    {\Lambda}_0:= \Pi_k f_0 + [\vha,\vhb] \in P_k(\T),\;\;
\Lambda_1:= \Pi_k f_1 \in  P_k(\cT; {\mathbb R}^2), \;\;
\Lambda_2 := \Pi_k f_2 - D^2_{\pw} \vha \in P_k(\cT; {\mathbb S})
\end{align*}
 The many orthogonalities \eqref{eqn:psi_def} of $\psi$ enter the final stage in two piecewise integration by parts for 
\begin{align}\nonumber
 \Lambda(\psi)
 %
  \equiv  \int_{\Omega} \big( \Lambda_0 \psi + \Lambda_1 \!\cdot \!\nabla \psi + \Lambda_2\!:\! D^2 \psi \big) \dx &=
  \sum_{E \in \E} \int_E \big( \psi \jump{\Lambda_1-\div_{\pw} \Lambda_2}_E\! \cdot\! \nu_E  + \nabla \psi\! \cdot \!\jump{\Lambda_2}_E \nu_E \big)\,\ds\\
  \label{eqn:algebraicidentity}
 &\; + \sum_{T \in \T} \int_T \big(  \Lambda_0 - \div_\pw \Lambda_1 + 
\div_\pw^2 \Lambda_2 \big)\, \psi\dx =0.
%
%
%
\end{align}
In fact, $\psi|_T \perp \Lambda_0- \div_{\pw} \Lambda_1+ \div^2_{\pw} \Lambda_2 \in P_k(T)$ in $L^2(T)$ for $T \in \T$, $\psi|_E \perp \jump{\Lambda_1-\div_{\pw} \Lambda_2}_E \in P_k(E) $ in $L^2(E)$ as well as $(\nabla \psi)|_E \perp \jump{\Lambda_2}_E \nu_E  \in P_k(E)^2 $ in $L^2(E)^2$ for all $E \in \E$ make each of the integrals vanish individually. 
Since $\zeta$ is the only element of $A\cap\omega(\zeta)$ by \eqref{eqn:single_load_assumption}, the properties of $\psi$ imply $\sum_{a\in A}\lambda_{a}\delta_{a}(\psi) = \lambda_{\zeta}$.
This, the algebraic identity \eqref{eqn:algebraicidentity}, and the first component $a(\ua,\psi) + \Gamma_1(\ua,\ub, \psi) = F(\psi)$ of the problem \eqref{vk_weak} (and~\eqref{VKE_weak}) with exact solution ${\bf u}=(\ua,\ub) \in \bV$ lead to 
\[ \lambda_{\zeta}= %
a_\pw(\ua-\vha,\psi)
+ \Gamma_{\pw,1}(\ua-\vha,\ub,\psi) + \Gamma_{\pw,1}(\vha, \ub-\vhb,\psi) + \Big(\Pi_kF+\sum_{a\in A}\lambda_{a}\delta_{a}-F\Big)(\psi). \]
%
A Cauchy inequality for $a_\pw$, the boundedness of $\Gamma_{\pw,1}$, and a routine estimation of the last term  as in \eqref{eqn:fbound} with the scaling $\|\psi\|_{H^s(T)}\leq h_{T}^{2-s}C_{\rm BH}\|\psi\|_{H^2(T)}$ for $s=0,1,2$ and $T\in\T(\zeta)$ from a Bramble-Hilbert lemma provide
\[ h_\zeta^{-1}  \etaz =|\lambda_\zeta| \le \trinl \psi \trinr
\Big(\big(1+\|\Gamma_{\pw,1}\|( \trinl \ub\trinr + \| \vha \|_h )\big) \| {\bf u}-{\bf v}_h \|_h + C_{\rm BH}{\rm osc}_k(F,\T)\Big). \]
The scaling $\trinl \psi \trinr \approx h_\zeta^{-1} $ and the boundedness of $\trinl \ub\trinr + \| \vha \|_h\leq \trb{{\bf u}}+\|{\bf v}_h\|_h$ by \eqref{eqn:vhbound} imply $\etaz \lesssim \| {\bf u}-{\bf v}_h \|_h+{\rm osc}_k(F,\T)$.
Since the set $|A\setminus\mathcal V|\lesssim 1$ is finite, the sum over all $\zeta\in A\setminus\mathcal V$ concludes the efficiency of $\mu(A\setminus\mathcal V) \lesssim \| {\bf u}-{\bf v}_h \|_h+{\rm osc}_k(F,\T)$.
Theorem \ref{thm:releff}.c and the quasi-optimality \eqref{quasioptimalsmootherP} of the smoother $P\equiv JI_\M$ provide the efficiency of  $\|[D^2v_h]_{\E}\tau_{\E}\|_{L^2(\E)}+j_h(v_h,v_h)^{1/2}$ for $v_h=\vha,\vhb$.
The efficiency of the other terms in $\boldsymbol{\sigma}(\T)$ does not follow verbatim, but a correction of standard (cubic volume and quadratic edge) bubble functions by a multiple of $\psi$ so that the resulting sum vanishes at $A$ decouples the contributions and leads to local efficiency as in \cite[Sec.~7.4]{CCBGNN22}.
\end{proof}

\section{Numerical experiments}%
\label{sec:Numerical experiments}
\input{sections/num_experiments}
\section*{Acknowledgements}
The research of the first two authors has been supported by the Deutsche Forschungsgemeinschaft in the Priority Program 1748
under the project \emph{foundation and application of generalized mixed FEM towards nonlinear problems
in solid mechanics} (CA 151/22-2).  This paper has been supported by the  SPARC project 
(id 235) {\it the mathematics and computation of plates} and SERB POWER Fellowship SPF/2020/000019.
The second author is also supported by the \emph{Berlin Mathematical School, Germany}.
\bibliographystyle{amsplain}
{\footnotesize{\bibliography{NSEBib,references}}}

